Semisimplicity criterion for 2-tonal partition algebras

We determine the semisimplicity criterion for even partition algebras over the complex field. Specifically we prove that the even/2-tonal partition algebras $P_n^2(\delta)$ over $\mathbb{C}$ are semisimple for all $n$ if and only if parameter $\delta \not\in \mathbb{N}_0$ .

==> tex/Pn-Brat-fig.tex <==

\begin{figure} 
\[
\includegraphics[width=12.8cm]{figs/PnBratelli8ii.eps}
\]
\caption{Augmented standard Bratelli diagram for $P_0 \subset P_1 \subset ...\subset P_4$. 
Vertices are standard modules with index as shown at the top of their column; and dimension shown in the box. Black edges indicate restriction rules (with multiplicities) so dimensions can be checked.
\textcolor{green}{Green} arrows indicate morphisms for $\delta=1 \in \C$
(see main text for commentary).
\textcolor{pink}{Pink} arrows indicate  morphisms for $\delta=2$.
(Morphisms for other $\delta$s 
%demoted to Figure~\ref{where???} 
omitted 
to avoid clutter.)
\label{fig:PnBratelli}}
\end{figure}




==> tex/Pn-case-1.tex <==



%% I have copied this section into a file for input,
%% in case we want to move it around.

%% NB in this file we later
%  \includegraphics[]{figs/PnBratelli8.eps}
%  \input{tex/examples-gram1}



\subsection{Gram matrices, tower representation theory and semisimplicity}
$\;$ 
\label{ss:gram-tower-semi}

\mdef 
Over $\C$ the algebras $P_n$ are generically semisimple, 
and in all cases with $\delta\neq 0$ the standard modules give a basis for 
the Grothendieck group,
so much of their combinatorial representation theory  %information 
is encoded in the standard restriction diagram 
(generically the Bratelli diagram, or else 
%(or 
a suitably enhanced version thereof)
for the tower of algebras 
$P_n \subset P_{n+1}$
in the generic case.
See Fig.\ref{fig:PnBratelli}.
In the figure we also record the morphisms between standard modules 
in the cases $\delta = 1,2$.


%\input{tex/Pn-Brat-fig}   %% promoted 



The Figure~\ref{fig:PnBratelli}  encodes a lot of information. However here we
will only need some specific observations from it.
Meanwhile, the gram matrices for the standard 
modules also contain a lot of information, but again 
we will only need parts of it, 
as in (\ref{de:Pn-spine}),
that are relatively readily accessible. 
To illustrate, we give some examples explicitly. 

%\ppm{[Demote gram-general.tex (was here ... to end of second Prop) to Appendix?? Saying:]}
{ For the reader desiring a review of the relevant gram matrix methods we include some generalities in 
\S\ref{ss:gramgen00} and 
\ca{Appendix~\ref{ss:appendb}.}}

%\input{tex/gram-general} %% promoted from P^2 section
\input{tex/examples-gram1}


\input{tex/gram-rep}


\mdef  \label{pa:gram-det-order}
The general $n$ form of the gram determinant 
$\det(\Gram_n(0))$
is somewhat non-trivial. But it is 
easy to see that the exponent of factor $\delta$ is 
the dimension of the module
(which is the Bell number $B(n)$ from (\ref{de:bell1})); 
and the total 
polynomial degree is 
$\sum_{l=1}^n l S(n,l) $ 
(coincidentally also dim$(\SSS_n((1)))$)
--- this is the sum of the exponents down the main diagonal, by the composition rule; 
and it is straightforward to check that this gives the highest order term in the Laplace expansion.

\mdef  \label{pa:simpleS0}
On the other hand we observe that the polynomial 
$\det(\Gram_n(0))$
must,
on representation theory grounds, 
contain factors as follows. 
(NB, we sometimes write $\SSS_n(0)$ for $\SSS_n(\emptyset)$ - purely for aesthetic reasons.)
The head of $\SSS_n(\lambda)$ 
when working over a field
depends on the specialisation $\delta\leadsto\delta_c$. For given $\delta_c$ we write $\DDD_n^{\delta_c}(\lambda)$ for the head.
For the factors $(\delta -1)$ in the determinant we observe that 
dimension of head of $\SSS_n(0)$ 
when $\delta_c =1$
is  $\dim(\DDD_n^{1}(0)) = 1$. 
We can observe this directly in our low rank 
diagram in Fig.\ref{fig:PnBratelli};
or in general by inspecting the Potts representation.
Thus the rank of the 
morphism (unique up to scalars, since necessarily head to socle) from 
standard module $\SSS_n(0)$ to 
costandard module $\nabla_n(0)$   %to standard 
is 1. 
The gram matrix $\Gram_n(0)$ intertwines these two modules over any ground ring.
By (\ref{eq:EPE}) it
always maps the head to the socle, % (see also \S\ref{ss:appendb}),
but its rank can
vary in specific specialisations (evalutations of $\delta$).
In order to have the right rank when $\delta=1$, 
it follows that all but one entry in the Smith form 
of $\Gram_n(0)$ over $\Z[\delta]$ (strictly speaking for a Smith form it should be over, say,
$\C[\delta]$, but here it makes no difference)
has a factor $(\delta -1)$.
%\ppm{[-say more about base change etc here???]}
So there are at least dim$(\SSS_n(0))$-1 such factors
in the determinant. 
That is, writing 
\beq  \label{eq:gram1} 
\det(\Gram_n(0)) = \prod_{\delta_c} (\delta-\delta_c)^{\alpha_{\delta_c}} 
\eq 
we have 
a bound on the exponent:
$\alpha_1 \geq \dim(\SSS_n(0))-1$.
A similar argument gives a bound 
\beq \label{eq:bound1}
\alpha_Q \geq \dim(\SSS_n(0))-\dim(\DDD_n^Q(0))
\eq 
on the number of
factors of each form $(\delta-Q)$ for $Q \in \N$. 
%The formula for $\dim(\DDD_n^Q(0))$ becomes more complicated. For example  
%$\dim(\DDD_n^2(0)) = 2^{n-1}$.
In general we have
\beq   \label{eq:dimD1} 
\dim(\DDD_n^Q(0))  \;=\; 
 \sum_{l=1}^{Q} S(n,l)
\eq 
arguing as in (\ref{pa:dimD0} - \ref{lem:basis1}). 
Hence
\[
\dim(\SSS_n(0))-\dim(\DDD_n^Q(0))  \;=\; 
\sum_{l=1}^n S(n,l) - \sum_{l=1}^{Q} S(n,l)
\; = \; \sum_{l=Q+1}^{n} S(n,l)
\]
Summing we obtain an overall bound for the polynomial degree
\[
%degree(\mbox{gram-det}) \; \geq \; 
degree(|\Gram_n (0) | )    \; \geq \; 
\sum_Q \sum_{l=Q+1}^{n} S(n,l) 
\; = \; \sum_{l=1}^n l S(n,l)
\]
%By a classical identity 
%\[ \dim(\SSS_n(1)) \; = \; \sum_{l=1}^n l S(n,l) 
%= ......
%\]   (and 
By 
our earlier observation in (\ref{pa:gram-det-order})
%)  %result)
this is saturated.
Thus the formulae (\ref{eq:bound1}) are equalities; and 
%In other words 
all factors in (\ref{eq:gram1}) come from 
these $Q$ values. Thus this gram determinant does not vanish for any other $\delta$ value. 
Thus $\SSS_n(0)$ is simple for all $n$ for all other $\delta$ values. 

\medskip

On the other hand we have the following. 

\mdef \label{pa:indicator}
\ignore{{ 
Finally we % observe 
argue
by Frobenius reciprocity 
%(arguing for example as in Cox {\em et al}'s method of {\em towers of recollement} \cite{cox2006representation}, %\cite{CoxMartinParkerXi06},
%%%\ppm{[-no! I don't think this alone is a helpful reference. Better to use \cite{MartinSaleur94b}]}
%and more specifically \cite{MartinSaleur94b})
using properties of the standard module restriction rules (as indicated in Fig.\ref{fig:PnBratelli} for example), 
that 
}}
%
If $\delta_c \neq 0$ and 
$\SSS_n(0)$ is simple for all $n$ then 
$P_n$ is semisimple for all $n$.

\medskip 

\newcommand{\ind}{Ind\;}
\newcommand{\res}{Res\;}
\newcommand{\mul}{\lambda}
\newcommand{\nul}{\nu}
%\newcommand{\bigplus}{{\huge{+}}}
\newcommand{\bigplus}{\sum} 
\newcommand{\lleadsto}{\mbox{\reflectbox{$\leadsto$}}}

We briefly recall the argument for this from \cite{MartinSaleur94b}, in preparation
for the 
modifications needed for the 
2-tonal case (which is in \ref{frecip}).
% 
%\footnote{

\noindent 
(I)
Suppose $n$ fixed. 
For brevity we assume the construction and basic properties of
the set $\SSS$ of standard $P_n$-modules $\SSS_n(\lambda)$ with 
$\lambda$ an integer partition of $l\leq n$. 
We write $|\lambda| = l$, as in (\ref{pa:globloc101}).

%In particular i
If a module $M$ has a filtration by a set ${\mathcal T}$ of modules we say that it has %an $\SSS$
a ${\mathcal T}$-filtration.
%}

\noindent
(II)
%Firstly n
Note that if $P_n$ is not semisimple then there must be a homomorphism
$\psi: \SSS_n(\mul) \rightarrow \SSS_n(\nul)$ for some 
distinct $\mul,\nul$;
in particular with $|\mul| > |\nul |$
(the latter condition comes from localisation functors and Maschke's Theorem,
considering (\ref{pa:globloc101})
and in particular (\ref{eq:uppertriangular});
or equivalently from quasiheredity).
And hence in particular some $\SSS_n(\nul) $ is not simple. 
So it is enough to prove that all $\SSS_n(\nul) $ are simple. 
We do this by induction on $|\nul|$.
\ignore{ 
Assuming $\delta \not\in \N_0$ then it 
is straightforward to eliminate cases with $|\mul| = |\nul | +1$,
so we consider $|\mul| > |\nul | +1$.
}

\noindent(III) 
%Consider
We will use the reciprocity 
\beq \label{eq:FR}
\Hom(\Ind \SSS_n(\mul), \SSS_{n+1}(\nul) ) \cong \Hom(\SSS_n(\mul) , \res \SSS_{n+1}(\nul) )
\eq 
where the $\Ind$ and $\res$ functors are those associated to 
the homomorphism $ P_{n} \hookrightarrow P_{n+1}$ given by 
$p \mapsto p\otimes 1$. 
By the usual $P_{n} \hookrightarrow P_{n+1}$ 
Induction/Restriction rules 
(as indicated,
at least at the level of characters, 
in Fig.\ref{fig:PnBratelli} for example), 
we have 
\beq \label{eq:Indres}
\Ind \SSS_n(\mul) \;\lleadsto  \;
%\bigplus_{\rho \in \mul\pm 1} \SSS_{n+1}(\rho) 
\{ \SSS_{n+1}(\rho) \; | \;    \rho \in \mul\pm \square   \}
,
\qquad \hspace{.21in} 
\res \SSS_{n+1}(\mul) \;\lleadsto  \; 
%\bigplus_{\rho \in \mul\pm 1} \SSS_{n}(\rho) 
\{ \SSS_{n}(\rho) \; | \;    \rho \in \mul\pm \square  \}
,
\eq 
where $\lleadsto {\mathcal T}$ indicates 
%$\SSS$
${\mathcal T}$-filtration; 
%and a covering set of  filtration factors; 
and $\lambda\pm\square $ indicates 
a set of factors 
adjacent to $\lambda$ in the Young graph (add or remove a box from the Young diagram, or add then remove), and hence 
with weights of rank between $|\lambda|+1$ and $|\lambda|-1$.
%So if we have $\psi: \SSS_n(\mul) \rightarrow \SSS_n(\nul)$ 
%then  ...
A schematic for this is:
\beq  \label{eq:FR111}
\includegraphics[width=10cm]{figs/FrobRecip111.eps}
\eq
where the brown walls partition the index set by increasing rank,
and the black lines indicate the factors of 
$\res\SSS_{n+1}(\mu)$ and $\Ind\SSS_n ( \lambda)$ respectively. 

\noindent
(IV)
So now suppose for an induction that modules 
$\SSS_n(\mu)$
of ranks $|\mu|$ up to $l$ are simple 
(for all $n$ - hence for fixed but arbitrary $n$).
The case we have %done above
concluded in (\ref{pa:simpleS0}) above - rank 0 - will 
eventually be the base of induction,
but for this proposition the base is exactly the hypothesis.
Excluding $\delta=0$ this implies no maps $\psi$ in
to $\SSS_n(\mu)$ (apart from self-isomorphism), 
so then in particular
for every $\mu$ of rank $|\mu| =l$ we have 
$\; \Hom(\Ind \SSS_n(\mul), \SSS_{n+1}(\mu) ) =0 \;$ 
for all $\mul$ of rank at least $|\mu|+2$, 
by 
the $\SSS$-module restriction rule from (\ref{eq:Indres}),
the upper-triangular simple decomposition matrix property
(\ref{eq:uppertriangular}), and Schur's Lemma.
But suppose (for a contradiction, in the inductive step to $l+1$) some 
$\SSS_n(\nu)$ with 
$\nu$ of rank $l+1$ 
is not simple, and hence has a map in, from $\SSS_n(\lambda)$ say. 
See the figure in (\ref{eq:FR111}).
The factors in any  %\ca
{$\res \SSS_{n+1}(\mu)$} as above are either in their own block by 
the inductive assumption, or of equal rank to $\nu$ and hence
(cf. (\ref{pa:globloc101}))
not involved
in extensions with $\SSS_n(\nu)$,
and for a suitable $\mu$ they include $\SSS_n(\nu)$. 
Thus there is a map in 
$  \Hom(\SSS_n(\mul) , \res \SSS_{n+1}(\mu) )  $. 
This then contradicts (\ref{eq:FR}). 
We deduce that every $\SSS_n(\nu)$ with 
$\nu$ of rank $l+1$ is simple, which completes the inductive step.

\medskip 


%\input{tex/semisimplicity}

\mdef 
Given (\ref{pa:indicator}) and (\ref{pa:simpleS0}) we have that $P_n$ is semisimple over $\C$
unless $\delta \in \N_0$. 

%as required,  %..., 
%and we are done.

\noindent 
(Cf. in particular the formulation of our Theorem~\ref{th:main} here.)



%\ppm{[FINISH ME! (...now it is essentially finished I think.)]}



%\input{tex/semisimplicity0}
%\input{tex/semisimplicity}





==> tex/Pn-case.tex <==

%% I have copied this section into a file for input,
%% in case we want to move it around.

%% NB in this file we later
%  \includegraphics[]{figs/PnBratelli8.eps}
%  \input{tex/examples-gram1}

\ignore{{ 

\subsection{How things work for the ordinary partition algebra}   $\;$ 

In this paper we follow the original method that works for
the partition algebras themselves.
In this subsection we assume familiarity with the partition algebra, and can then give a convenient brief overview of our approach in terms of the partition algebra case.

}}



\subsection{\ppmm{Basic representation theory}} \label{ss:brt}
%\ppm{[-just trying a new subsection to see if organisation is better. - would plan to move \ref{pa:globloc101} here, after the modular stuff. Move done now.]}

\newcommand{\Cdelta}{\C[\delta_c\in \C]} % C as Zd-alg

Recall that the partition algebras $P_n$ 
(for $n \in \N$)
may be defined over $\Z[\delta]$, where they are of finite rank; and hence over any ring that is a $\Z[\delta]$-algebra, by base change.
For example we can work over the ring $\C[\delta]$, 
which is a $\Z[\delta]$-algebra by inclusion; 
or over $\C$ by evaluating
$\delta$ as some element $\delta_c\in\C$
(we may write   % $\C[\delta\in \C]$ 
$\Cdelta$ 
for $\C$ made a $\Z[\delta]$-algebra in this way, 
for example $\C[2]$,
or simply write $\C$ if no ambiguity arises, leaving the action of $\delta$ implicit). 

\ppmx{[just around here is where the standard modules are defined. this is one of the things that we will parallel for the tonal case, so perhaps this should be highlighted more clearly - so that explicit reference to this part can be made later. - and then explicitly paralleled in the tonal case. (BTW, I note that here it says very explicitly that qh will not be used.)]}

Indeed 
the pair 
$(\C[\delta],  \Cdelta )$
represent a modular system for the 
representation theory of 
$P_n(\delta_c\in\C)$ - the algebra over 
$ \Cdelta $.    %the latter.

\mdef \label{lem:ss01}
Over the field of fractions of 
%the former
$\C[\delta]$
these algebras $P_n$ are semisimple. 
The simple modules can be labeled with $\lambda\in \Lambda^n$, the set of integer partitions of ranks up to $n$
(see \ref{pa:globloc102}).
There are integral lattice forms
of the simple modules,
a preferred choice of 
which 
(see \ref{pa:globloc102})
thus define
{\em standard modules} 
over $\Z[\delta]$, and hence by base change over any ground ring.
%
$\;$ \confer{\ref{pa:Pn2mod}}

%\newcommand{\DDD}{{\mathcal{D}}}  %% simple module.
%%%^promoted to Pmacros.tex

Once the ground ring is fixed, the standard modules may be 
denoted $\SSS_n(\lambda)$, where label $\lambda$ is an integer partition of rank up to $n$.
Over $\C[\delta]$ these modules are quotients of indecomposable projectives.
Upon specialisation to $\delta_c \in \C^\times$ they have  %with 
pairwise distinct simple heads.
%provided that we localise at $\delta$.
%The simplest example 
We write $\DDD_n^{\delta_c}(\lambda)$ for the simple head of $\SSS_n(\lambda)$  in the specialisation evaluating $\delta$ at $\delta_c$. 

\medskip 

%\mdef 
%%(
{\it{Remark}}: Here we use the language of classical Brauer modular representation theory (see e.g. Curtis--Reiner \cite{CurtisReiner62}). 
The modules $\SSS_n(\lambda)$ 
also coincide with cellular cell modules and quasi-hereditary standard modules but we will not need this technology.
A natural construction is via the partition category
over the corresponding ground ring, which we briefly recall below.
%%)


\ppmx{[could perhaps put \ref{pa:globloc101} here for example. Done.]}

\input{tex/Pn-repthy}  %% moved from sec.2


\newcommand{\E}{E}

\medskip 
\mdef   \label{de:Pn-spine} 
%%For 
%It will be convenient to review a simple example. 
Fix $n$  and a ground field $k$ (with the property of $\Z[\delta]$-algebra).
%Consider  the partition basis of $P_n$ --- the set $\rmP_n$ of set partitions of two rows of $n$ vertices.
Let $\E_1 =\bb{n}$  %denote the partition in the partition basis of $P_n$ 
%%(set partitions of two rows of $n$ vertices)
%in which there is only one part
%(denoted $\bb{n}$ when $n$ is not fixed, 
as in (\ref{bn}) above. 
And let %$E_0$ denote the partition, hence partition basis element, 
%in which the top row of $n$ vertices are one part, and the bottom row another part:
\beq   \label{eq:E0} 
\E_0 = \bbb{n}  = \{ \{1,2,...,n\},\{1',2',...,n'\}\}
\eq 
We  have $\E_0 \E_0 = \delta \E_0$, 
and 
\beq \label{eq:EPE} 
\E_0 P_n \E_0 = \delta k \E_0 ,
\eq 
Thus $\E_0$ passes to an unnormalised primitive idempotent in any specialisation for which $\delta$ has an inverse.
In these cases then, the left ideal $P_n \E_0$ and right ideal $\E_0 P_n$ are  indecomposable projective. 
In fact $\SSS_n(\emptyset) = P_n \E_0$; and 
$\SSS_n((1)) = P_n \E_1 / P_n \E_0 P_n$. 
%We have a
By (\ref{eq:EPE}) we have a 
multiplication map
%bilinear form 
%$\kappa : P_n \E_0 \times \E_0 P_n \rightarrow k$
$\mu :  \E_0 P_n \times P_n \E_0  \rightarrow k\E_0$
and then a map $\kappa :  \E_0 P_n \times P_n \E_0  \rightarrow k$
given by 
%$(a,b) \mapsto \kappa(a,b)$ where 
$\mu(a,b)=ab = \kappa(a,b) \E_0$. 
Observe that this gives a contravariant form on $P_n \E_0$
with respect to the usual flip map. 

Recall the chain of ideals
$P_n \supset P_n E_1 P_n \supset P_n E_0 P_n$.
We immediately have $E_1 E_1 = E_1$ and 
$E_1 P_n E_1 = k E_1$ mod. $P_nE_0 P_n$.
Thus $E_1$ is a primitive idempotent in the corresponding quotient. 
%
\confer{\ref{de:Pn2-spine}}



\newcommand{\Gram}{\Gamma}

\mdef 
\label{de:PnE0basis}
Observe that $P_n E_0$ has basis the subset of the partition basis of $P_n$ consisting of all partitions in which the bottom row of vertices exactly make one of the parts. The basis is thus constructed by taking all partitions of the top row of $n$ vertices. 
There is a corresponding `flipped' basis for $\E_0 P_n$,
and with these bases we fix a gram matrix $\Gram_n(\emptyset)$ for the form $\kappa$. 
(See also \S\ref{ss:gramgen00}.)

\mdef 
Later it will be convenient to organise the top-row partitions 
in the partition basis of $P_n \E_0$ 
according to the number of parts.
There is of course one with one part, for any $n$. 
The partitions into two parts or less are 
double-counted by   %in bijection with 
the power set of the set of vertices, so there are $2^{n-1}$ of these. 
For the three parts case, and higher cases, things are a bit more complicated, and we will return to these shortly. 


\subsection{Potts functors, symmetry and simple modules} 
$\;$   \label{ss:PottsFunctors}

\ppm{[maybe move this section to the end of \S\ref{ss:constructPd}?]}

%% following now in
%%
%\input{tex/Pmacros}
%%
%\newcommand{\Potts}{{\mathfrak{P}}}
%\newcommand{\Pcat}{{\mathsf{P}}}
%\newcommand{\Mat}{{\mathsf{Mat}}}
%\newcommand{\mat}{\left( \begin{array}{ccccccccccccc}}
%\newcommand{\tam}{\end{array} \right)}

\noindent 
This is an opportune moment to consider the Potts functors (see e.g. \cite{Martin91}), 
which facilitate the analysis of key representations that we will need. 

\mdef   \label{de:PottsFunctor}
%This is an opportune moment to consider the Potts functors (see e.g. \cite{Martin91}). 
%
For a given commutative ring $\Fk$, 
$\Mat$ denotes the monoidal category of matrices over $\Fk$ with Kronecker product as monoidal product. 
%
For fixed $Q \in \N$,
$\Pcat(Q)$ 
(or $\Pcat$) 
denotes the partition category with $\delta_c = Q$
as in (\ref{de:Pcat}).
%
For fixed $Q \in \N$ 
the Potts functor is a strict monoidal functor 
$$
\Potts : \Pcat(Q) \rightarrow \Mat   .
$$
%, where $\Pcat(Q)$ is the partition category with $\delta_c = Q$, and $\Mat$ the monoidal category of matrices over $k$ with Kronecker product as monoidal product.  
The functor may be given as follows.



%\input{tex/Pcat}

\mdef 
The category $\Pcat$ 
is linearly-monoidally generated by the unique partition elements in 
$\Pcat(1,0)$ and $\Pcat(0,1)$; the single-part elements in $\Pcat(1,2)$ and $\Pcat(2,1)$;
and the elementary permutation element in 
$\Pcat(2,2)$. 

The image under $\Potts$ of the generating object 1 is $Q$.
So the image of an element in $\Pcat(i,j)$ lies in $\Mat(Q^i, Q^j)$.
The rows of a matrix in $\Mat(Q^i, Q^j)$ are indexed by words in 
$\ul{Q}^i  \cong \hom(\ul{i}, \ul{Q})$;
and the columns by words in $\ul{Q}^j$. 
The images for $Q=2$ of the generators above are
\beq   \label{eq:Potts1}
\Potts(\{\{1\}\}) = \mat 1\\1 \tam
\hspace{1.8in}   %\] \[
\Potts(\{\{1'\}\}) = \mat 1 & 1 \tam
\eq 
\beq 
\Potts(\{\{1,1',2'\}\}) = 
\mat 
 1&0&0&0 \\ 
0&0&0&1\tam
\hspace{1.358in}   
%\] \[
\Potts(\{\{1,2,1'\}\}) = 
%\mat 1&1&1&1 \\ 1&1&1&1 \tam
\mat 1&0\\
0&0 \\ 
0&0\\
0&1
 \tam
\hspace{.3in} 
\eq 
\beq  \label{eq:Potts12}
\Potts(\{\{1,2'\},\{2,1'\}\}) = 
\mat 
1&0&0&0 \\ 
0&0&1&0 \\ 
0&1&0&0 \\ 
0&0&0&1 \tam
\eq 

%...

In other words,
noting that each matrix entry position corresponds to a $Q$-state Potts configuration (or $Q$-colouring) on the corresponding vertex set, 
all vertices in the same part must have the same `colour' for an entry 1, otherwise the entry is 0.
(The ``Potts rule''.) 


\mdef Examples. Derived from (\ref{eq:Potts1})-(\ref{eq:Potts12}) above, 
keeping $Q=2$, we have 
(with $T$ for transpose) 
\beq 
\Potts(\{1,2,...,n\}) = \mat
1&0&0&...&0&0&1   \tam^T 
\eq 
\beq 
\Potts(\{1,2,...,n,1'\}) = \mat
1&0&0&...&0&0&0 \\  0&0&0&...&0&0&1   
\tam^T 
\eq 
\ignore{{ 
%We have 
With the basis ordered as 111,112,121,122,211,212,221,222, we have
\beq 
\Potts(\{\{1\},\{2\},\{3\}\}) = \mat
1&1&1&1&1&1&1&1
\tam ,
\hspace{1cm}
\Potts(\{\{1,2\},\{3\}\}) = \mat
1&1&0&0&0&0&1&1
\tam ,
\eq 
}}


\mdef  \label{pr:SWdual01}
Observe that the functor 
$\Potts(Q)$ is invariant under the diagonal action of 
the symmetric group
$\Sym_Q$
%\ppm{[-where is symm gp first introduced here?? - it is now already mentioned in the first para of this section.]}
(the element $\sigma_1 \in \Sym_Q$ takes word $w=11..1$ to 
$\sigma_1 w =22..2$ and so on). 
This is simply the Potts symmetry \cite{Martin91}, 
but in algebraic terms,
%That is, 
for $(\sigma)$ the matrix form of an element in $\Sym_Q$, and $p \in \Pcat(n,m)$ 
\beq  \label{eq:SW00}
\mat \sigma \tam^{\otimes n} \Potts(p) 
\; = \; \Potts(p)  \mat \sigma \tam^{\otimes m}
\eq 

\mdef The examples of (\ref{eq:SW00}) that we will use concern $p\in \rmP_{\ul{n}}$.
For example, with $Q=2$ and for any partition $p$ of $\ul{n}$ we have 
$$
\mat 0&1 \\ 1&0 \tam^{\otimes n} \Potts(p) 
\; = \; \Potts(p)  \mat 0&1 \\ 1&0 \tam^{\otimes 0}
\; = \; \Potts(p) 
$$
and so in particular 
the vector entry $\Potts(p)_{11..1}$ obeys 
$\; \Potts(p)_{11..1} = \Potts(p)_{22..2}$.

\mdef  \label{lem:norbits}
In light of the $\Sym_Q$ invariance, 
the dimension of the image of $\Pcat(n,0)$ under $\Potts$ is thus 
bounded above  %given 
by the number of orbits of the $\Sym_Q$ action on $\ul{Q}^n$.

We will see that this number is the 
number of partitions of $\ul{n}$ into at most $Q$ parts,
%cardinality of  ...
and that the bound is saturated. 



\medskip 


\mdef 
\label{pa:dimD0}
In $P_n(Q)$ 
%Here 
the idempotent form of
the partition
$E_0$ is $\frac{1}{Q} E_0$ and $Trace(\Potts(E_0)) =Q$. % so we
We deduce that the simple head of the left module 
$P_n E_0 \cong \Pcat(n,0) $ 
occurs exactly once as a summand of the Potts representation 
$\Potts(P_n = \Pcat(n,n))$. 

\mdef  \label{pa:2bas}
Indeed for $Q=2$ it 
%will be clear 
is straightforward to see 
that the $2^{n-1}$ basis elements of $P_n E_0$  corresponding to 
(up to) two-part partitions have independent images in $\Potts$; and that elements of higher order then do not.
Thus the dimension of the simple head is $2^{n-1}$. 

\newcommand{\cruder}{<}

\ignore{{ 
For example consider the three-part partition 
$q= \{\{1\},\{2\},\{3\}\}$.
In general we write $p \cruder p'$ 
to mean that $p$ is a 
cruder partition than $p'$.
Thus 
$ \{\{1,2\},\{3\}\} \cruder  \{\{1\},\{2\},\{3\}\} $  
and so on.

%while (with the basis ordered as 111,112,121,122,211,212,221,222) we have 
%$\Potts(\{\{1,2\},\{3\}\}) = \mat
%1&1&0&0&0&0&1&1 \tam , $
$
\Potts(\{\{1,3\},\{2\}\}) = \mat
1&0&1&0&0&1&0&1
\tam ,
$
$
\Potts(\{\{2,3\},\{1\}\}) = \mat
1&0&0&1&1&0&0&1
\tam .
$
So  %%, with $q= \{\{1\},\{2\},\{3\}\}$, 
$$
\Potts(q) \; - \; 
\sum_{p < q} %%\{\{1\},\{2\},\{3\}\}} 
\left( \Potts(p) -\sum_{p'<p} \Potts(p') \right)
\;=\; \mat 
0&0&0&0&0&0&0&0
%1&1&1&1&1&1&1&1
\tam 
$$
%%(where $p<q$ means $p$ is a finer partition than $q$).

%%Thus the dimension of the simple head is $2^{n-1}$. 
}}

\medskip

To illustrate this, and the generalisation to all $Q$ that we will use, 
we first introduce a bit more notation.


\mdef  \label{pa:(123)}
We may  %- here we 
follow \cite[Ch.8]{Martin91} in writing $(12)(3)$ for the set $\{ \{1,2\},\{3\}\}$, and so on, just to avoid curly-bracket overload.


\mdef 
%Let us 
Recall we 
write $\Pcat_{ij}$ for the partition basis of 
the morphism set $\Pcat(i,j)$
(later we may abbreviate $\Pcat_{nn}$ as $\Pcat_n$).
Thus there is a unique element in each 
$\Pcat_{ij}\siz_1$. 
And $\;\Pcat_{n0}\siz_2  \;\cup\;  \Pcat_{n0}\siz_1 $ 
yields the basis of 
the image under $\Potts$  of 
$P_n E_0  \cong \Pcat(n,0)$  in (\ref{pa:2bas}) above
%(under $\Potts$ 
(when $Q=2$),
noting (\ref{de:PnE0basis}).  % and (\ref{pa:2bas}). 
%(ignoring for the moment the contribution from $\Pcat_{0n}\siz_1$).

Example:
\beq  \label{eq:P123}
\Pcat_{30}\siz_1 = \{   (123)  \}
,\qquad 
\Pcat_{30}\siz_2 = \{   (12)(3), (13)(2), (1)(23)  \}
,\qquad 
\Pcat_{30}\siz_3 = \{   (1)(2)(3)  \}
\eq 



\mdef 
For any set $S$ a function $f:S\rightarrow T$ to any target defines an equivalence relation, and hence a partition 
$\varpi(f)$
of $S$, by $a\sim b$ if $f(a)=f(b)$.
Thus in particular there is a partition $\varpi(w)$ of $\ul{n}$ for every word 
$w$ in $\ul{Q}^n$. 
For example $\varpi(112)=(12)(3)$. 

Observe that 
the image of the map $ \varpi : \ul{Q}^n    \; \rightarrow \;\; \rmP_{\ul{n}} \; $
is $\; \sqcup_{i=1}^Q \; \rmP_{\ul{n}} \siz_i $. That is, 
$$
\varpi : \ul{Q}^n    \; \rightarrow \;\;  \sqcup_{i=1}^Q \; \rmP_{\ul{n}} \siz_i 
$$
is  well-defined and surjective. 


\mdef \label{lem:orb1}
Observe here that the set $\varpi^{-1}(\varpi(w))$ is the orbit of $w$ under the diagonal $\Sym_Q$ action as in (\ref{pr:SWdual01}). 
For example, when $Q=2$, 
$\varpi^{-1}((12)(3)) = \{ 112, 221 \}$;
and 
when $Q=3$,  
$\varpi^{-1}((1234)) = \{ 1111, 2222, 3333  \}$
and
$\varpi^{-1}((12)(3)(4)) = \{ 1123, 1132, 2213, 2231, 3312, 3321  \}$.

We can choose representatives for the orbits by using dictionary order.
Fixing $Q$ and $p \in \sqcup_{i=1}^Q \; \rmP_{\ul{n}} \siz_i  $,
let us write $\varpi^- (p)$ for the representative in $\varpi^{-1}(p)$. 
For example $\varpi^- ((12)(3))=112$.


\mdef  \label{eg:123}
Considering the partitions of $\ul{3}$ organised as in (\ref{eq:P123}) 
we have
\beq \label{eq:123}
\Potts((123)) = \mat 1 &0& 0& 0& 0&0&0&1  \tam^T 
, \qquad 
\eq 
\beq  
\Potts((12)(3)) = \mat 1 &1& 0& 0& 0&0&1&1  \tam^T 
= \mat 1&0&0&1 \tam^T \otimes \mat 1&1 \tam^T 
\eq 
In fact this is the first instance so far in which the Kronecker convention in $\Mat$ is relevant to how we write the image.
Here we say that the possible states of vertices 123 in the $Q=2$ state case are ordered as 111, 112, 121, 122, 211, 212, 221, 222.
(All other cases will be clear from this.)
This is sometimes called aB convention since in writing $A\otimes B$ the first block we write is given  by $B$ multiplied by the first entry of $A$. 

We also have
\[
\Potts((13)(2)) = \mat 1 &0& 1& 0& 0&1&0&1  \tam^T 
, \qquad
\] \beq \label{eq:1-23} 
\Potts((1)(23) = \mat 1 &0& 0& 1& 1&0&0&1  \tam^T
= \mat 1&1 \tam^T \otimes \mat 1&0&0&1 \tam^T
\eq 
Clearly these (\ref{eq:123}-\ref{eq:1-23}) are all independent of each other. 
Meanwhile 
$$
\Potts((1)(2)(3)) = \mat 1&1&1&1&1&1&1&1 \tam^T 
$$
is not then also independent. 

\mdef
Example with $Q=3$. The states of vertices 123 in case $Q=3$ are
given by
$\ul{3}^3 = $ 
\\  $\mbox{ }$  $\;$ \hspace{-.321in} 
$\{ \!\!\!\!$
{\tiny{ 
111, 112, 113, 121, 122, 123, 131, 132, 133, $\;$
211, 212, 213, 221, 222, 223, 231, 232, 233, $\;$ 
311, 312, 313, 321, 322, 323, 331, 332, 333. 
}}  $\!\!\!\!\!\!\}$
\\ 
The orbits of the diagonal action of $\Sym_3$ are \quad 
111, 222, 333, \qquad
112, 113, 221, 223, 331, 332, \qquad 
121, 131, 212, 232, 313, 323, \qquad
122, 133, 211, 233, 311, 322, \qquad
123, 132, 213, 231, 312, 321.
\\
Thus we only need to give the five vector entries in a transversal of this partition to give any $\Potts(p)$.  

Representatives of orbits in $\ul{3}^5$ (243 words altogether)
can be organised according to integer partitions of 5 into at most 3 parts
((5), (41), (32), (311), (221)). %; and
A complete list of representatives
are: 
11111,  \qquad 
11112, 11121, 11211, 12111, 21111,  \qquad 
11122, 11212, 11221, 12112, 12121, 12211, 21112, 21121, 21211, 22111, \qquad 
11123, 11213, 11231, 12113, 12131, 12311, 21113, 21131, 21311, 23111, \qquad 
11223, 11232, 11322, 12123, 12132, 13122, 12213, 12312, 13212, 
12231, 12321, 13221, 31122, 31212, 31221.
Note, one in an orbit of size 3 and 40 in orbits of size 6 --- a 41d space.
Of course these correspond to the 41 set partitions of $\ul{5}$ of size at most 3.

Thus to give $\Potts((1)(2)(3)(45))$ we only need to give $\Potts(p)_w$
for $w$ in the lists above. For example 
$\Potts(p)_{11111} =1$; $\Potts(p)_{11112} =0$, 
$\Potts(p)_{11121} =0$, $\Potts(p)_{11211} =1$ and so on.  




\mdef 
Let $S$ be any given set, and $p,q \in \rmP_S$. 
Write $p \prec q$ 
(or $q \succ p$)
to denote that partition $p$ is less refined than $q$.
%E.g.
For example
$(123)\prec (12)(3) \prec (1)(2)(3)$.
Note that this gives a partial order on $\Pcat_S$. % for any set.

\mdef   \label{lem:basis1}
Observe that $\Potts(\varpi(w))_w =1$ (recall words $w$ index vector elements here, cf. (\ref{pr:SWdual01})). 
And observe that for every %less-refined 
partition $q\nsucceq \varpi(w)$ we have $\Potts(q)_w =0$.
This verifies the independence of the set of 
images of 
partitions into at most $Q$ parts.
But 
with (\ref{lem:orb1}) 
it also yields that the images of these partitions form a spanning set,
taking account of the diagonal action of $\Sym_Q$.
\\
Specifically in our example (\ref{eg:123}) above we have 
$\varpi^{-1}((123))=\{111,222\}$, 
$\varpi^{-1}((12)(3))=\{112,221\}$, 
$\varpi^{-1}((1)(23))=\{122,211\}$, 
$\varpi^{-1}((13)(2))=\{121,212\}$, 
whose union is $\ul{2}^3$, so $\Potts((1)(2)(3))$ must be {\em dependent}.
%But also it yields that $\Potts(p) = 0$ for a partition of more than $Q$ parts.




\mdef 
Aside:
Observe in the  % above 
`Potts rule' 
(see (\ref{de:PottsFunctor}))
that 
different parts may have different
colours, but of course if there are only two colours then if there are more than two parts some of them will have the same colour, and potentially be indistinguishable from cruder partitions. 
We deduce that $\Potts$ has a significant kernel.
%In particular ...

Consider in particular the representation of $P_n(Q)$ given by $\Potts$. 
This is a representation on $(\C^Q)^{\otimes n}$, and hence of dimension $Q^n$.
Furthermore the image is a *-algebra and hence a semisimple quotient of $P_n(Q)$.
Indeed the corresponding quotient tower gives a Jones basic construction 
in the sense, for example, of \cite{GoodmanDelaharpeJones89}
(in fact two such).

\newcommand{\ff}{{\mathsf{f}}} %% Young antisymm 

An example of an element in the kernel is the 
unnormalised Young antisymmetrizer of rank $Q+1$
(in $P_n$ for any $n>Q$ by the natural inclusion). 
We write this for now as 
$\ff_{Q+1} = \sum_{g \in S_n} (-1)^{len(g)} g$. 
For example $\ff_2 = (11')(22') - (12')(21')$.
Evidently this vanishes in $\Potts$ when $Q=1$. 
More generally the image of $\ff_{Q+1}$ vanishes whenever we have symmetry under the exchange of two vertices among $Q+1$ - which holds in $\Potts$ for any element of $P_n$ since we only have $Q$ colours with which to distinguish vertices.


\mdef
%Observe also 
We have seen 
that the partition category action commutes with the action of the symmetric group $\Sym_Q$ permuting the `colours' 
(as opposed to the vertices)
- the diagonal action on the corresponding tensor spaces. 
This is the Potts symmetry (of the Potts model). 
Indeed these actions are in (an appropriate generalisation of) Schur--Weyl duality. 



\subsection{Gram matrices, tower representation theory and semisimplicity}
$\;$ 
\label{ss:gram-tower-semi}

\mdef 
Over $\C$ the algebras $P_n$ are generically semisimple, 
and in all cases with $\delta\neq 0$ the standard modules give a basis for 
the Grothendieck group,
so much of their combinatorial representation theory  %information 
is encoded in the standard restriction diagram 
(generically the Bratelli diagram, or else 
%(or 
a suitably enhanced version thereof)
for the tower of algebras 
$P_n \subset P_{n+1}$
in the generic case.
See Fig.\ref{fig:PnBratelli}.
In the figure we also record the morphisms between standard modules 
in the cases $\delta = 1,2$.


\begin{figure} 
\[
\includegraphics[width=12.8cm]{figs/PnBratelli8.eps}
\]
\caption{Augmented Bratelli diagram for $P_0 \subset P_1 \subset ...\subset P_4$. 
Vertices are standard modules with index as shown at the top of their column; and dimension shown in the box. Black edges indicate restriction rules (with multiplicities) so dimensions can be checked.
\textcolor{green}{Green} arrows indicate morphisms for $\delta=1 \in \C$
(see main text for commentary).
\textcolor{pink}{Pink} arrows indicate  morphisms for $\delta=2$.
(Morphisms for other $\delta$s 
%demoted to Figure~\ref{where???} 
omitted 
to avoid clutter.)
\label{fig:PnBratelli}}
\end{figure}

The Figure encodes a lot of information. However here we
will only need some specific observations from it.
Meanwhile, the gram matrices for the standard 
modules also contain a lot of information, but again 
we will only need parts of it that are relatively readily accessible. 
To illustrate, we give some examples explicitly. 

%\ppm{[Demote gram-general.tex (was here ... to end of second Prop) to Appendix?? Saying:]}
{ For the reader desiring a review of the relevant gram matrix methods we include some generalities in 
\S\ref{ss:gramgen00} and 
Appendix~\ref{ss:appendb}.}

%\input{tex/gram-general} %% promoted from P^2 section
\input{tex/examples-gram1}


\mdef The gram matrix $\Gram_n(0)$ intertwines $\SSS_n(0)$ with its contravariant dual.
The modules are generically isomorphic so the intertwiner is invertible
in generic specialisations.
But for $\delta=1$ we see from Fig.\ref{fig:PnBratelli} that $\Gram_2(0)$ 
has a 1d submodule, so the intertwiner maps the 1d head to the socle, and so has
rank 1 on evaluation at $\delta = 1$.
%%\ppm{[intertwine example?]}  DONE!

\input{tex/gram-rep}


\mdef  \label{pa:gram-det-order}
The general $n$ form of the gram determinant is somewhat non-trivial. But it is 
easy to see that the exponent of factor $\delta$ is 
the dimension of the module
(which is the Bell number $B(n)$ from (\ref{de:bell1})); 
and the total 
polynomial degree is 
$\sum_{l=1}^n l S(n,l) $ 
(coincidentally also dim$(\SSS_n((1)))$)
--- this is the sum of the exponents down the main diagonal, by the composition rule; 
and it is straightforward to check that this gives the highest order term in the Laplace expansion.

\mdef  \label{pa:simpleS0}
On the other hand we observe that the polynomial 
$\det(\Gram_n(0))$
must,
on representation theory grounds, 
contain factors as follows. 
(NB, we sometimes write $\SSS_n(0)$ for $\SSS_n(\emptyset)$ - purely for aesthetic reasons.)
The head of $\SSS_n(\lambda)$ 
when working over a field
depends on the specialisation $\delta\leadsto\delta_c$. For given $\delta_c$ we write $\DDD_n^{\delta_c}(\lambda)$ for the head.
For the factors $(\delta -1)$ in the determinant we observe that 
dimension of head of $\SSS_n(0)$ 
when $\delta_c =1$
is  $\dim(\DDD_n^{1}(0)) = 1$. 
We can observe this directly in our low rank 
diagram in Fig.\ref{fig:PnBratelli};
or in general by inspecting the Potts representation.
Thus the rank of the 
morphism (unique up to scalars, since necessarily head to socle) from 
standard module $\SSS_n(0)$ to 
costandard module $\nabla_n(0)$   %to standard 
is 1. 
The gram matrix $\Gram_n(0)$ intertwines these two modules over any ground ring.
By (\ref{eq:EPE}) it
always maps the head to the socle (see also \S\ref{ss:appendb}),
but its rank can
vary in specific specialisations (evalutations of $\delta$).
In order to have the right rank when $\delta=1$, 
it follows that all but one entry in the Smith form 
of $\Gram_n(0)$ over $\Z[\delta]$ (strictly speaking for a Smith form it should be over, say,
$\C[\delta]$, but here it makes no difference)
has a factor $(\delta -1)$.
%\ppm{[-say more about base change etc here???]}
So there are at least dim$(\SSS_n(0))$-1 such factors
in the determinant. 
That is, writing 
\beq  \label{eq:gram1} 
\det(\Gram_n(0)) = \prod_{\delta_c} (\delta-\delta_c)^{\alpha_{\delta_c}} 
\eq 
we have 
a bound on the exponent:
$\alpha_1 \geq \dim(\SSS_n(0))-1$.
A similar argument gives a bound 
\beq \label{eq:bound1}
\alpha_Q \geq \dim(\SSS_n(0))-\dim(\DDD_n^Q(0))
\eq 
on the number of
factors of each form $(\delta-Q)$ for $Q \in \N$. 
%The formula for $\dim(\DDD_n^Q(0))$ becomes more complicated. For example  
%$\dim(\DDD_n^2(0)) = 2^{n-1}$.
In general we have
\beq   \label{eq:dimD1} 
\dim(\DDD_n^Q(0))  \;=\; 
 \sum_{l=1}^{Q} S(n,l)
\eq 
arguing as in (\ref{pa:dimD0} - \ref{lem:basis1}). 
Hence
\[
\dim(\SSS_n(0))-\dim(\DDD_n^Q(0))  \;=\; 
\sum_{l=1}^n S(n,l) - \sum_{l=1}^{Q} S(n,l)
\; = \; \sum_{l=Q+1}^{n} S(n,l)
\]
Summing we obtain an overall bound for the polynomial degree
\[
%degree(\mbox{gram-det}) \; \geq \; 
degree(|\Gram_n (0) | )    \; \geq \; 
\sum_Q \sum_{l=Q+1}^{n} S(n,l) 
\; = \; \sum_{l=1}^n l S(n,l)
\]
%By a classical identity 
%\[ \dim(\SSS_n(1)) \; = \; \sum_{l=1}^n l S(n,l) 
%= ......
%\]   (and 
By 
our earlier observation in (\ref{pa:gram-det-order})
%)  %result)
this is saturated.
Thus the formulae (\ref{eq:bound1}) are equalities; and 
%In other words 
all factors in (\ref{eq:gram1}) come from 
these $Q$ values. Thus this gram determinant does not vanish for any other $\delta$ value. 
Thus $\SSS_n(0)$ is simple for all $n$ for all other $\delta$ values. 

\medskip

On the other hand we have the following. 

\mdef \label{pa:indicator}
\ignore{{ 
Finally we % observe 
argue
by Frobenius reciprocity 
%(arguing for example as in Cox {\em et al}'s method of {\em towers of recollement} \cite{cox2006representation}, %\cite{CoxMartinParkerXi06},
%%%\ppm{[-no! I don't think this alone is a helpful reference. Better to use \cite{MartinSaleur94b}]}
%and more specifically \cite{MartinSaleur94b})
using properties of the standard module restriction rules (as indicated in Fig.\ref{fig:PnBratelli} for example), 
that 
}}
%
If $\delta_c \neq 0$ and 
$\SSS_n(0)$ is simple for all $n$ then 
$P_n$ is semisimple for all $n$.

\medskip 

\newcommand{\ind}{Ind\;}
\newcommand{\res}{Res\;}
\newcommand{\mul}{\lambda}
\newcommand{\nul}{\nu}
%\newcommand{\bigplus}{{\huge{+}}}
\newcommand{\bigplus}{\sum} 
\newcommand{\lleadsto}{\mbox{\reflectbox{$\leadsto$}}}

We briefly recall the argument for this from \cite{MartinSaleur94b}, in preparation
for the 
modifications needed for the 
2-tonal case (which is in \ref{frecip}).
% 
%\footnote{

\noindent 
(I)
Suppose $n$ fixed. 
For brevity we assume the construction and basic properties of
the set $\SSS$ of standard $P_n$-modules $\SSS_n(\lambda)$ with 
$\lambda$ an integer partition of $l\leq n$. 
We write $|\lambda| = l$, as in (\ref{pa:globloc101}).

%In particular i
If a module $M$ has a filtration by a set ${\mathcal T}$ of modules we say that it has %an $\SSS$
a ${\mathcal T}$-filtration.
%}

\noindent
(II)
%Firstly n
Note that if $P_n$ is not semisimple then there must be a homomorphism
$\psi: \SSS_n(\mul) \rightarrow \SSS_n(\nul)$ for some 
distinct $\mul,\nul$;
in particular with $|\mul| > |\nul |$
(the latter condition comes from localisation functors and Maschke's Theorem,
considering (\ref{pa:globloc101})
and in particular (\ref{eq:uppertriangular});
or equivalently from quasiheredity).
And hence in particular some $\SSS_n(\nul) $ is not simple. 
So it is enough to prove that all $\SSS_n(\nul) $ are simple. 
We do this by induction on $|\nul|$.
\ignore{ 
Assuming $\delta \not\in \N_0$ then it 
is straightforward to eliminate cases with $|\mul| = |\nul | +1$,
so we consider $|\mul| > |\nul | +1$.
}

\noindent(III) 
%Consider
We will use the reciprocity 
\beq \label{eq:FR}
\Hom(\Ind \SSS_n(\mul), \SSS_{n+1}(\nul) ) \cong \Hom(\SSS_n(\mul) , \res \SSS_{n+1}(\nul) )
\eq 
where the $\Ind$ and $\res$ functors are those associated to 
the homomorphism $ P_{n} \hookrightarrow P_{n+1}$ given by 
$p \mapsto p\otimes 1$. 
By the usual $P_{n} \hookrightarrow P_{n+1}$ 
Induction/Restriction rules 
(as indicated,
at least at the level of characters, 
in Fig.\ref{fig:PnBratelli} for example), 
we have 
\beq \label{eq:Indres}
\Ind \SSS_n(\mul) \;\lleadsto  \;
%\bigplus_{\rho \in \mul\pm 1} \SSS_{n+1}(\rho) 
\{ \SSS_{n+1}(\rho) \; | \;    \rho \in \mul\pm \square   \}
,
\qquad \hspace{.21in} 
\res \SSS_{n+1}(\mul) \;\lleadsto  \; 
%\bigplus_{\rho \in \mul\pm 1} \SSS_{n}(\rho) 
\{ \SSS_{n}(\rho) \; | \;    \rho \in \mul\pm \square  \}
,
\eq 
where $\lleadsto {\mathcal T}$ indicates 
%$\SSS$
${\mathcal T}$-filtration; 
%and a covering set of  filtration factors; 
and $\lambda\pm\square $ indicates 
a set of factors 
adjacent to $\lambda$ in the Young graph (add or remove a box from the Young diagram, or add then remove), and hence 
with weights of rank between $|\lambda|+1$ and $|\lambda|-1$.
%So if we have $\psi: \SSS_n(\mul) \rightarrow \SSS_n(\nul)$ 
%then  ...
A schematic for this is:
\beq  \label{eq:FR111}
\includegraphics[width=10cm]{figs/FrobRecip111.eps}
\eq
where the brown walls partition the index set by increasing rank,
and the black lines indicate the factors of 
$\res\SSS_{n+1}(\mu)$ and $\Ind\SSS_n ( \lambda)$ respectively. 

\noindent
(IV)
So now suppose for an induction that modules 
$\SSS_n(\mu)$
of ranks $|\mu|$ up to $l$ are simple 
(for all $n$ - hence for fixed but arbitrary $n$).
The case we have %done above
concluded in (\ref{pa:simpleS0}) above - rank 0 - will 
eventually be the base of induction,
but for this proposition the base is exactly the hypothesis.
Excluding $\delta=0$ this implies no maps $\psi$ in
to $\SSS_n(\mu)$ (apart from self-isomorphism), 
so then in particular
for every $\mu$ of rank $|\mu| =l$ we have 
$\; \Hom(\Ind \SSS_n(\mul), \SSS_{n+1}(\mu) ) =0 \;$ 
for all $\mul$ of rank at least $|\mu|+2$, 
by 
the $\SSS$-module restriction rule from (\ref{eq:Indres}),
the upper-triangular simple decomposition matrix property
(\ref{eq:uppertriangular}), and Schur's Lemma.
But suppose (for a contradiction, in the inductive step to $l+1$) some 
$\SSS_n(\nu)$ with 
$\nu$ of rank $l+1$ 
is not simple, and hence has a map in, from $\SSS_n(\lambda)$ say. 
See the figure in (\ref{eq:FR111}).
The factors in any  %\ca
{$\res \SSS_{n+1}(\mu)$} as above are either in their own block by 
the inductive assumption, or of equal rank to $\nu$ and hence
(cf. (\ref{pa:globloc101}))
not involved
in extensions with $\SSS_n(\nu)$,
and for a suitable $\mu$ they include $\SSS_n(\nu)$. 
Thus there is a map in 
$  \Hom(\SSS_n(\mul) , \res \SSS_{n+1}(\mu) )  $. 
This then contradicts (\ref{eq:FR}). 
We deduce that every $\SSS_n(\nu)$ with 
$\nu$ of rank $l+1$ is simple, which completes the inductive step.

\medskip 


%\input{tex/semisimplicity}

\mdef 
Given (\ref{pa:indicator}) and (\ref{pa:simpleS0}) we have that $P_n$ is semisimple over $\C$
unless $\delta \in \N_0$. 

%as required,  %..., 
%and we are done.

\noindent 
(Cf. in particular the formulation of our Theorem~\ref{th:main} here.)



%\ppm{[FINISH ME! (...now it is essentially finished I think.)]}



%\input{tex/semisimplicity0}
%\input{tex/semisimplicity}




==> tex/WPW-P-schema.tex <==

%\ppm{[15/8/24: maybe move \ref{pa:globloc2}-\ref{pa:Trep}-... to here - in sec.5 - now?]}\ca{[both are now here]} %%thank you.
%%% ppm: since then I decided to try a different place for this. (maybe returning even?!)  %%%

\newcommand{\WW}{W^2}
\newcommand{\WWW}{W_b^2}
\newcommand{\oWW}{\overline{W}^2}
\newcommand{\oWWW}{\overline{W}_b^2}

\mdef  \label{pa:globloc2}
We will  % need 
use a version of (\ref{pa:globloc101}) for $P^2_n$. $\;$
%%%Recall from \cite{amm2019tonal} that 
%For given $n \geq 2$, note that $\WW$  from (\ref{pa:U}) is in $P^2_n$. 
For given $n$ note that $\WW$ and  $\WWW$ from (\ref{pa:U}) are in $P^2_n$ (these require $n\geq 2$ and $n\geq 3$ respectively).
Note that $\WWW$ is idempotent, and 
if $\delta$ is invertible $\WW$ is also preidempotent. 
\ppmx{[fixed now?: -this seems false at the moment! shall we define $\W$ as $\W_n$ in the cases $n>2$? ...Could define it as $\U$ in case $n=2$, and point out that this is not idempotent! - although this seems ugly!]}
%and is in $P^2_n$. 
Recall then for example from \cite{amm2019tonal} that 
%and that 
$\WW P^2_n \WW \cong P^2_{n-2}$;
and that the quotient algebra
$
A^2_n = P^2_n / P^2_n \WW P^2_n
$
is semisimple over $\C$ - see in particular 
\cite[(9.3)]{amm2019tonal}. 
\\
In  \cite[(9.3)]{amm2019tonal}   %where 
we see also that the same identities hold replacing $\WW$ with 
$\WWW$, or $\oWW$, or $\oWWW$. 
\ca{For example, the following figure schematically indicates,
for $n=7$, 
the isomorphism between $W^2_b P^2_7(\delta)W^2_b$  and $P^2_5(\delta)$ (a similar figure appears in \cite[\S7.1]{amm2019tonal}).}
\beq \label{eq:wpw} 
\rb{-.22in}{\ig[width= 10cm]{wwpw.eps}}
\eq \beq 
\rb{-.22in}{\ig[width= 10cm]{wwpwn.eps}}
\eq 




==> tex/abkmp-defsV2.tex <==

\noindent 
%In particular 
In this paper 
$\N$ denotes the natural numbers and $\N_0$ the natural numbers with 0. 
%%[Chwas, Have I got this right?????]} 
%
%Here t
The symmetric group is denoted $\Sym_n$. 
We write $\omega_n$ for the Coxeter longest-word element in $\Sym_n$. 

In this Section we follow    %%\cite{amm1,
\cite{amm2019tonal} almost exactly,
apart from adding some appropriate fresh examples
(we reproduce some constructions here simply for convenience of reference).
%\\ { } 
%[-is this true? If so, we should say so. If not, we should explain why.]}\ca{[yes, it is true, as you say we do so to set up the notation.]}


\medskip 

{For given ground % field 
ring $\Fk$,
and $\nk \in \N_0$,}
let $P_\nk(\delta)$ be the usual Partition algebra with parameter $\delta \in \Fk$.
We assume familiarity with these algebras (see e.g. \cite{Martin94,Halverson05})
and the corresponding partition category $\Pcat(\delta)$ 
(again as in \cite{Martin94}, or for example \cite{Martin08a}).
We will define $\PP$ as a subalgebra, in (\ref{de:P2}).

Here we will fix the ground field to $\C$,
unless stated otherwise
(much of our exposition works for arbitrary $\Fk$, 
but not all of the representation theory, 
and for the latter steps below a different approach would be needed even for $\Fk$  an arbitrary field).

%\newcommand{\rmP}{{\mathsf P}} %% set of set partitions
%%\newcommand{\rmPe}{{\mathsf P}^e} %% set of even set partitions
%\newcommand{\rmPe}{{\mathsf P}^{(e)}} %% set of even set partitions

\mdef  \label{pa:Pn}
If $S$ is a set, we write $\rmP_S$ for the set of set partitions of $S$. 
%We write $\rmPe_S$ for the subset of $\rmP_S$ of set partitions where every part is of even size.
Consider a set consisting of 
$n+m$ nodes, 
organised as
an `upper' row of $n$ nodes and a lower row of $m$ nodes.
We label the upper nodes, left to right, 
%of the diagram 
using the set 
$\underline{n} = \{1,2,\dots,n\}$; 
and the lower row similarly by 
$\underline{m}' = \{1',2',\dots,m'\}$. 

We write $\rmP_{n,m}$ 
(or $\rmP_{nm} $ if $nm$ is unambiguous)
for the set of all set partitions of the above set.
%(which we can write as 
That is, 
$\rmP_{n,m} = \rmP_{ \underline{n} \cup \underline{m}' } $. 
%). 
Of course this is essentially the same as the set of set partitions of any set of size $n+m$.

%Observe 
Recall 
that $\rmP_n := \rmP_{n,n}$ 
can be taken as
the defining basis of the algebra $P_\nk(\delta)$. 
The morphism sets 
of the partition category $\Pcat(\delta)$ are 
$\Pcat(\delta)(i,j) = \Fk \rmP_{i,j}$. 
As noted, we assume familiarity with the category composition
(which, when $i=j=n$, is the algebra composition).

%\input{tex/Pcat}

\newcommand{\bb}[1]{b^{#1}}  %% the 1-part partition in rank n
\newcommand{\bbb}[1]{b_0^{#1}}  %% the 1-part partition in rank n
\newcommand{\w}[1]{w^{#1}}

\mdef  \label{exa:ww}
Examples and notations. 
For $l \in \N$ 
let $\w{l} = \{ \{1,2,...,l \}\}  \in \rmP_{l,0}$ and 
$\w{l*} = \{ \{1',2',...,l' \}\} \in \rmP_{0,l}$
(for given $l$ these are written simply $\w{}$ and $\w{*}$ in \cite[(2.4)]{amm2019tonal}). 
These are composable in the category:
$\w{l} \w{l*} = \{\underline{l}, \underline{l'} \}$
and
$\w{l*} \w{l} = \delta \emptyset \; \in \Fk \rmP_{0,0}$.
Let 
$
\;\U \; :=\;  \w{2} \w{2*} \; = \; \{\{1,2\},\{1',2'\}\}   \in \rmP_{2,2}  %.
$
(in \cite[(2.2)]{amm2019tonal} this is denoted $u$). 
Let 
$ \;  \bb{l} \; := \;
\{\underline{l} \cup \underline{l'} \} $
%\ppm{[-should use $l$ not $n$ here; -should explain why changing, and recall notation from...]}
(as in \cite[(2.2)]{amm2019tonal})
and 
$\; \bbb{l} := \; \w{l} \w{l*} \; = \; 
\{\underline{l} , \underline{l'} \} 
\;  \; \in\rmP_{l,l} $. 


\mdef 
An element of $\rmP_{n,m}$ can be represented 
as a graph (graph edges  %indicating
yielding connected components and hence parts);
and hence
pictorially
as a graph drawn 
in a box with the rows of nodes 
$\{ 1,2,...,n\}$ 
on the top and 
$\{ 1',2',...,m'\}$
on the
bottom edge of the box,
%; and the graph edges indicating connected components, 
as for example here:
\beq 
\qquad 
\{\{ 1,2,6,6'\},\{ 3,4 \}, \{ 5,3'\}, \{ 1',2'\},\{ 4',5'\}\} 
\; = \; 
\rb{-.21in}{\ig[width=3cm]{exatonal.eps}}
\in \rmP_{6,6}
\eq 
Observe that drawn graph edges can cross in the interior of the box, but must do so transversally
to avoid ambiguity.
 $\; $ %\\
%Then 
Even more schematically we have pictures/diagrams such as:
\beq\label{bn} 
\bb{n} \; 
%:= \; \{\underline{n} \cup \underline{n'} \} 
\; = \; 
\rb{-.21in}{\ig[width=3cm]{exaschem.eps} }\in\rmP_{n,n}
%...... picture ............
\eq
%\ppm{[-different colour for box and graph?]}
%--- for given $n$ this example would represent the partition with only a single part.

Of course, such pictorial representations are highly non-unique.
There are many graphs representing the same partition; and many embeddings for each graph.
We can even allow some representative graphs with additional vertices 
(drawn in the interior of the box), so long as the connections among 
$\underline{n} \cup \underline{n'} $  are correct. 
We give  %more
several examples later. 


\mdef 
Let $p\in\rmP_{\nk,m}$. 
An element $s\in p$ is called a {\em part} or {\em block}.
A part is called a {\em propagating part} if it consists of nodes from both the upper and lower row. 

For example, the partition 
\rb{-.21in}{\ig[width=3.5cm]{exapropag.eps}}$\;\in\rmP_{8,8}$ 
has 3 propagating parts and 4 non-propagating parts.
%\ppm{[-partition??]}

\mdef \label{de:flip}
The flip map $-^* : \rmP_{i,j} \rightarrow \rmP_{j,i}$ is obtained by toggling the prime label
on vertices (thus flipping diagrams from top to bottom). 
For example $\{\{1,2,1'\},\{2'\}\}^* = \{\{1,2',1'\},\{2\}\}$;
and see also (\ref{exa:ww}).
Note that this extends linearly to take the algebra to its opposite (and also the category). 

Observe that there is a natural inclusion 
of the symmetric group
$\Sym_n \hookrightarrow P_n(\delta)$. 
For $p \in \rmP_{n,m} $
the map $p \mapsto \omega_n p \omega_m  \in \rmP_{n,m}$,
denoted $p \mapsto \overline{p}$ 
corresponds to {\em left-right} flip of a diagram for $p$. 

\mdef  \label{pa:U}
Observe that side-by-side concatenation of diagrams gives a map
$\otimes : \rmP_{i,j} \times \rmP_{k,l} \rightarrow \rmP_{i+k,j+l}$.
This extends to a monoidal product on category $\Pcat(\delta)$. 
%
For example %, defining $\U = \{\{1,2\},\{1',2'\}\}   \in \rmP_{2,2}$, then 
\beq 
\U \otimes \U \; = \; 
\{\{1,2\},\{1',2'\}\} \otimes \{\{1,2\},\{1',2'\}\} 
\; = \;
\{\{1,2\},\{1',2'\}, \{3,4\},\{3',4'\} \}  \; \in \rmP_{4,4} 
\eq 
%Define $\U = \{\{1,2\},\{1',2'\}\}   \in \rmP_{2}$.
Then 
$\U^{\otimes m} \in \rmP_{2m,2m}$. 

\newcommand{\W}{{\mathcal W}} %% partition
\newcommand{\A}{{\mathcal A}}  %% partition 
\newcommand{\one}[1]{1^{#1}}  %% partition

If we write 1 for a partition we mean 
$1=\{\{1,1'\}\}$. 
Then $\one{n} = 1\otimes 1 \otimes ...\otimes 1$ ($n$ factors). 
(In \cite{amm2019tonal} this $\one{n}$ is denoted $1_n$.)  
%
As in \cite[(3.8)]{amm2019tonal} we have, for given $n$,
%elements $W^l  , W^l_b  \in \rmP_{n,n}$  given by
\[
W^l \; := \; \left( \w{l} \w{l*}  \right) \otimes \one{n-l}
\; \in \; \rmP_{n,n},
\hspace{.9cm}
W_b^l \; \; := \;  b^{l+1}   \otimes 1^{n-l-1}
\; \in \; \rmP_{n,n}   ,
\hspace{.9cm}
\overline{W}_b^l \; \; = \;   1^{n-l-1}   \otimes b^{l+1}  
%\; \in \; \rmP_{n,n}
\]
%(see (\ref{pa:U}) for the $\otimes$ product and $1_{n-l}$)
%(in \cite{amm2019tonal} $\one{n}$ is denoted $1_n$).  
%\ppm{[-need to move this. - DONE. but for now just trying to get things fixed in notation for use later!!!]}



%Here, for fixed $n>2$ let 
%$\W = b^2 \otimes 1^{n-2}$ 
%\beq\label{Wn} 
%\W_n \; 
%%:= \; \{\underline{n} \cup \underline{n'} \} 
%\; = \; 
%\rb{-.21in}{\ig[width=3cm]{Wn.eps} }\in\rmP_{n,n}
%...... picture ............
%\eq
%and for  $n=2$  let %$\W_2=\U.$
%\ppm{[-what is going on here??! Can you remind me why we have such a strange mix of definitions? In (\ref{pa:globloc2}) we say $\W$ is idempotent, and use it, so some fix is needed.]}
%The above $\W_n$ (for $n>2$) 
%equates  %seems to be related 
%to $W_b^2$
%the case $l=2$ of 
%$$    W_b^l \; \;= \;  b^{l+1}   \otimes 1^{n-l-1}   $$ 
%from \cite[(3.8)]{amm2019tonal}.  
%\ppm{[right? why is $\W_2$ different?]}


%\ca{[I think this should be $\W_n = \left(b^3 \otimes 1^{n-3}\right)\left(\U \otimes 1^{n-2}\right)\left(b^3 \otimes 1^{n-3}\right)$ for 2.11 \ref{pa:globloc2} to work]}\ppm{[-I have not understood this yet!]}.
For given $n>0$ let 
$\A_1 \; := \; \{\{1\},\{1'\}\}\otimes 1^{n-1} =W^1$.



==> tex/abkmp22.tex <==

\subsection{%Algebra f
Filtration of algebra $P_\nk^\dell(\delta)$ by ideals} $\;$ 

Here we continue with tonality $\dell$ a fixed positive integer. 

\mdef \label{de:hashi}
Let $p\in\rmP_\nk^\dell$, 
and $1\leq i\leq d$.
A propagating part $s\in p$ is \emph{co}-$i$ if the restriction of  $s$ to the underlying set of the upper row has order $i$ $\mod d$.

For each $i$ we define
$$\#^i(p) := \mbox{ number of blocks in $p$ which are co-$i$.}
$$
%\ppm{ %[-where is this notation defined??? ]
%[ Why so many problems here????? copy from earlier paper?????? or at least stay closer to it?]}\ca{[I agree, it should be better now]}

\mdef 
The \emph{propagating vector}  of a partition $p \in \rmP_n^\dell$ 
%\ppm{[--???! no!]}\ca{[i think it should be $\rmP_n^\dell$ since we have only defined the co-i for $\dell$-tonal partitions]}
is defined to be:
$$
\#\bar{\ }(p) \; := \; (\#^1(p), \#^2(p), \ldots, \#^\dell(p))    \; \in \; \N_0^d .
$$
%\ppm{[-something wrong here!]}\ca{[it should be correct now.]}

\noindent 
Examples: 
\\
 For $\dell=2$, we have $\#\bar{\ }(1_n)=(n,0)$; 
 
\ignore{{ 
as noted in ????? we have 
\beq \label{eq:P29ex} 
\rb{-.22in}{\ig[width= 4.5cm]{exapropvect.eps}}
\;\; \in \;\; \rmP^2_{9}
\eq 
}}

\noindent 
For the partition $p$  as in (\ref{eq:P29ex}) we have, from (\ref{de:hashi}), 
$$
\#^1(p) = \ca{3} , \qquad 
\#^2(p) = 1.
$$
So,
$$
\#\bar{\ }(\rb{-.12in}{\ig[width= 2.5cm]{exapropvect.eps}})=(3,1)  .
$$
%\ppm{[-definitely does not agree with the above. I am lost.]}\ca{[I think I fixed the issue]}


\mdef
%\ppm{For $\dell\in ...$ and $n\in ...$} 
For positive integers $d$ and $n$
define a subset of $\N_0^\dell$ by 
$$
\gamma^{\dell,n}:= 
\left\{ \vec{m} \in \N_0^\dell \mid \left(n - \sum_{i=1}^\dell im_i
\right)/\dell \in \N_0 \right\}
$$
%For $\vec{m} \in \gamma^{\dell,\nk}$ let
%$$
%r_{\vec{m}} =\sum_{i=1}^\dell im_i 
%\qquad
%$$ 
Let $\{e_1,e_2,\dots,e_\dell\}$ be the standard basis for the free $\Z$-module $\Z^\dell$. Define  $\mathsf{X}_\dell\subset \Z^{\dell}$ by 
\[\mathsf{X}_\dell:=\{e_k-e_i-e_j\mid 1\leq i,j,k\leq \dell\text{ and }i+j=k\mod\dell\}.\]
Then $(\gamma^{\dell,\nk},\leqslant)$ is a finite poset where $\vec{m}'\leqslant \vec{m}$ if $\vec{m}- \vec{m}'$ is in the nonnegative integral span of $\mathsf{X}_\dell$. See \cite{amm1} for the combinatorial properties of the poset $(\gamma^{\dell,\nk},\leqslant)$.


\mdef
For $d=2$ \ppmm{and fixed (sufficiently large) but arbitrary $n$ and ${\vec{m}}\in  \gamma^{\dell,2}$
we define $ a^{\vec{m}} \in \rmP^2_\nk$ by}
\begin{equation}
    \label{eq:a def} 
a^{\vec{m}} =a^{(m_1,m_2)}= \rb{-.45in}{\ig[width=7cm]{am.eps}}
\end{equation} 
If we want to focus on the value of $\nk$ we can write
$a^{\vec{m}} = a_\nk^{\vec{m}} $.
For example 
$$
\rmP^2_{16} \ni a_{16}^{(4,4)} =
\rb{-.21in}{\ig[width=6.5cm]{amexa.eps}}$$




\mdef\label{2.9}\ca{[I think we can safely delete all \ref{2.9} ]}
\ppm{[-really! don't we use $w$ later!?!?]}
\begin{equation}
a^{\vec{m}} = \otimes_i
  (b^i)^{\otimes m_i} \otimes (ww^*)^{\otimes (k-r_{\vec{m}}) /\dell}=a^{(m_1,m_2)}
\end{equation} 
where $b^i$ is the diagram 
\ppm{partition}
with $i$ top nodes and $i$ bottom nodes which
are all in the same block, \ca{$w \in P^\dell(\dell,0)$ has $\dell$} nodes on the top
which are all linked.
\ppm{[-obviously there is still a lot of work to do fixing all this.]}

$$
b^i = \rb{-.21in}{\includegraphics{bi.eps}}
\qquad  \hspace{1cm}
w=\rb{-.21in}{\includegraphics{wr.eps}}
$$



\mdef 
Note $\#^{\bar{\ }}(a_{\vec{m}}) = \vec{m}$.

\mdef  
We set
%\ppm{[is this the right font!?-]}
$
\rmP^{\vec{m}}_\nk = \{ p \in \rmP_\nk^\dell \mid \#^{\bar{\ }}(p) = \vec{m}\}
$.

$$
\rmP_\nk^\dell\ni W = ww^* \otimes 1_{n-\dell} = 
\rb{-.21in}{\includegraphics{WW.eps}} 
\; \in \; 
\mathfrak{S}_{\dell} a^{(n-\dell, 0 ,\ldots, 0)}
\mathfrak{S}_{\dell}
$$
\ppm{[-point to where this last is defined? it looks like it is after!!]}

\ppm{[section is called filtration by ideals. where does this happen?][- moved the next subsection start to start to address this. OK? still doesn't do filtration.]}

\medskip 





%\subsection{The standard modules of $P^2_\nk(\delta)$}  $\;$

\mdef 
For a given $\Vec{m}=(m_1,m_2)\in \gamma^{2,\nk}$, %let 
consider the double-sided ideal
\beq  \label{eq:dsiI}
I^{<\Vec{m}}
\; = \;
\sum_{\Vec{m}'<\Vec{m}}
P^2_\nk(\delta) \; a^{\vec{m}'}P^2_\nk(\delta)
\; ,\eq  
where is $a^{\vec{m}}$ defined in (\ref{eq:a def}).
%\ppm{[-where is $a$ defined in (\ref{eq:a def})?]}\ca{[Yes, thank you]}
Then let
$$
P_\nk^{\vec{m}}=P^2_\nk(\delta)/I^{<\Vec{m}} .
$$ 
be the corresponding quotient algebra. 



\subsection{The standard modules of $P^2_\nk(\delta)$}
$\;$


For $r$ a positive integer, let $\Sym_r$ denote the symmetric group on $r$ letters. 
\ppm{[-shall we say this earlier?]}
For $\vec{m}$ 
\ppm{$\in \N_0^2$ [???]}
as in (\ref{???}),
let $\Sym_{\vec{m}}=\Sym_{m_1}\times\Sym_{m_2}$.
Let
$\C[\Sym_{\vec{m}}]$ denote the group algebra of $\Sym_{\vec{m}}$ over $\C$. %\ppm{[-explain notation]}

\mdef 
By \cite[Lemma~5.7]{amm2019tonal} there is an isomorphism of $\C$-algebras \begin{equation}
     a^{\vec{m}}P_\nk^{\vec{m}}a^{\vec{m}}\cong \C[\Sym_{\vec{m}}] 
 \end{equation}
Note that this isomorphism depends on $\delta$. \ppm{[-depends on $\delta$?]}

Consequently, when $\delta\neq0$ an indexing set 
$\Lambda(P^2_\nk(\delta))$
for the simple modules %, $\Lambda(P^2_\nk(\delta))$,  
of $P^2_\nk(\delta)$ is given by  (see \cite[Theorem 5.9]{amm2019tonal})  
\begin{equation}
    \Lambda(P^2_\nk(\delta))=\bigsqcup_{\vec{m}\in \gamma^{2,\nk}}\Lambda(\C[\Sym_{\vec{m}}])
\end{equation} 
where 
$\Lambda(\C[\Sym_{\vec{m}}])$ 
is a suitable indexing set for the simple modules of $\C[\Sym_{\vec{m}}]$,
such as we will recall shortly.
\\
When $\nk$ is even and $\delta=0$, the above equation overcounts the simple modules of $P^2_\nk(0)$. In  this case $\Lambda(P^2_\nk(0))=\bigsqcup_{\vec{m}\in \gamma^{2,\nk}\setminus\{\vec{0} \}}\Lambda(\C[\Sym_{\vec{m}}]).$

\mdef 
Let $m$ be a nonnegative integer. A sequence of positive integers $ \lambda=(\lambda_1, \lambda_2,\dots ,\lambda_q)$ is a partition of $m$, written $\lambda\vdash m$, if $|\lambda|=\sum_{i=1}^{q} \lambda_i=m$ and $\lambda_1\geq\lambda_2\geq\dots\geq\lambda_q$.
Note that $\emptyset$ is the only partition of 0. 
We also write $(\lambda,\mu)\vdash m$ if $\lambda$ and $\mu$ are integer partitions and $|\lambda|+|\mu|=m.$
\\For each $\vec{m}=(m_1,m_2)\in \gamma^{2,\nk}$ we have 
\begin{equation}
    \Lambda(\C[\Sym_{\vec{m}}])=\{(\lambda,\mu)\mid \lambda\vdash m_1\text{ and }\mu\vdash m_2 \}.
\end{equation}
 Let $(\lambda, \mu)\in \Lambda(P^2_\nk(\delta))$, we write $\Sym_{(|\lambda|, |\mu|)}$ for $\Sym_{|\lambda|}\times\Sym_{|\mu|}$. 
 
\mdef 
 There exists a primitive idempotent $e_{(\lambda, \mu)}$ in the group algebra $\C[\Sym_{(|\lambda|, |\mu|)}]$ such that the left ideal \begin{equation}
    \mathtt{Sp}_{(\lambda, \mu)}=\C[\Sym_{(|\lambda|, |\mu|)}]e_{(\lambda, \mu)}
\end{equation} is a ``Specht" module, 
see e.g.  \cite{curtis1962representation,james1978representation}. 

\mdef\label{glob} 
For any $\vec{m}\in \gamma^{2,\nk}$ there is an exact functor 
\begin{equation}
    G_{\vec{m}}: \C[\Sym_{\vec{m}}]\text{-mod}\longrightarrow P_\nk^{\vec{m}}\text{-mod}
\end{equation}
defined by $G_{\vec{m}}M=P_\nk^{\vec{m}} a^{\vec{m}}\otimes_{\Sym_{\vec{m}}}M$. 
In particular, we set 
$$
\cell_\nk(\lambda, \mu):=G_{\vec{m}}\mathtt{Sp}_{(\lambda, \mu)}
.$$ 


\begin{thm}\cite[Theorem 9.7]{amm2019tonal}
 Let $\delta\in\C^\times$
 {and $\nk \in \N$}. 
 For all but finitely many values of $\delta$ we have:
 \begin{enumerate}
     \item[I)] $\{\cell_\nk(\lambda, \mu)\mid (\lambda, \mu)\in \Lambda(P^2_\nk(\delta))\}$ forms a complete set of simple modules of $P^2_\nk(\delta)$
     up to isomorphism.
     \item[II)] $P^2_\nk(\delta)$ is semisimple. 
     {\qed}
 \end{enumerate}
\end{thm}

\mdef 
In particular, $\cell(\emptyset, \emptyset)$ (when $\delta\neq0$) and $\cell((1), \emptyset)$ are indecomposable projective modules.


\mdef\label{S(0,0)} 
A basis 
%\ppm{[-what does this mean?  just basis maybe? or basis of partitions? or as left ideal of something??]}\ca{[I fixed it, thank you]}
of each $\cell_\nk(\lambda, \mu)$ is given in \cite{amm2019tonal}. 

\mdef 
$\cell_n(\emptyset, \emptyset)$  %(when $\delta\neq0$)
and $\cell_n((1), \emptyset)$ 
%and 
possess partition basis, as given below.
\ppm{[???]}
If  $\nk$ is an even integer then  $\cell_\nk(\emptyset,\emptyset)$ has a partition basis 
\begin{equation} \label{eq:block-even} 
\begin{split}
&\{p\in \rmP_\nk^2\mid \#\bar{\ }(p)=(0,0)\text{ and } \underline{n}'\in p\}\\=&
\{q\cup\{\underline{n}'\}\mid q\text{ is a partition of }\underline{n}\text{ into blocks of even size}\}. 
\end{split}
\end{equation}

\ppm{[-does this work. my guess is this is not quite an ideal, so either fix the primed bit or omit it (plays no role up to isomorphism???]}\ca{[How about the new version? I think here we don't need it to be an ideal, left ideal is enough]}

When $n$ is odd, a partition basis of $\cell_\nk((1), \emptyset)$ is given by
$$\{p\in \rmP_\nk^2\mid \#\bar{\ }(p)=(1,0)\text{ and there is a part }s\in p\text{ with } \underline{n}'\subset s\}$$
Note that, for each basis element $p$ of $\cell_\nk((1), \emptyset)$, we have $pb_n=p$, where $b_n$ is the partition defined in \eqref{bn}.





==> tex/gram-general.tex <==


\medskip 

\ppm{[We need to introduce this section properly!][...but we are just going to delete it now, right?]}
We continue with algebra $A$ as in \S\ref{ss:gramgen00}. %(\ref{where?}). 
Here for any $A$-module $M$ we write $M^o$ for its contravariant (cv) dual with respect to a given opposite-isomorphism.

\medskip 


\ignore{{ 
The modules for which we compute gram matrices here have  a unique cv form on them, up to scalars.
More generally, 
\ca{For a given $R$-module \ppm{[$A$-module?]} $M$ there might be more than one contravariant form on it and showing that one of them is non-singular does not guarantee the simplicity of $M$. 
\ppm{[-perhaps this is a strange way to say it here? Of course for an arbitrary module there could be many forms. Why is this worth remarking here? ...Probably this question will be fixed by the exposition to be added at the start of the subsection.]}
However, the  following proposition provides a sufficient condition for which to prove $\spine$ is simple it is enough to show that 
the form 
$\langle-,-
\rangle_{e_{(\emptyset,\emptyset)}}$ is non-singular}.
}}


\begin{prop}\label{nonsingular}\cite[Proposition 2.7e]{green2007polynomial}
     Let $K$ be a field, and $A$ be a $K$-algebra with a given involutive
antiautomorphism. 
(I) Let $M$ and $N$ be two left $A$-modules. Then
    for each contravariant form 
    $\langle-,-\rangle:M\times N\to K$ 
    we associate  
    $\psi\in Hom_A(M,N^o)$ such that $\psi(m)(n)=\langle m,n\rangle$. This association is a bijection between such forms and morphisms. 
\\ (II)   
Any given such form is non-singular if and only if the corresponding $\psi$ is an isomorphism.
\qed 
\end{prop}

\ignore{{ 
% \ppm{[isnt this just a corrolary of A.1??  Delete it??]}
%Further, i
If $M= N$ 
%and} satisfies the conditions of Proposition~\ref{dimL=rank}, 
then there is a
unique 
cv form 
$\langle-,-\rangle:M\times M\to K$
up to scalars, 
%\ppm{[-regardless of $N$? Or $N=M$?]}
and the form is non–singular 
iff the associated $\psi$ is an isomorphism 
(in particular it is non–singular if $M=N$ is simple). 
%\qed 
%\end{prop} 
}}


\medskip 

Under suitable conditions (which we have seen apply in our case) we have existence
and uniqueness up to scalars:

\newcommand{\Mo}{M_-}

\begin{prop}\label{dimL=rank}
     Let $K$ be a field, and $A$ be a $K$-algebra with a given involutive
antiautomorphism.   %, say ${(-)}^o$.
Let $M$ be an $A$-module. 
Suppose (I) $M$ has a unique maximal proper submodule (call it $\Mo$) and
hence simple head $L = M/\Mo$; 
(II) composition factor $L$ has multiplicity one in $M$; and
(III) $L\simeq L^o$.
%\ppm{[-how do we know this in our application? we do know it, but we haven't said.]}
%\ppm{[-where defined?] (here for any module $M$ we write $M^o$ for its contravariant dual with respect to a given opposite-isomorphism)}. %% I have pushed this def above now.
Then  $\dim Hom_A(M, M^o)=1$ and $\psi\in Hom_A(M, M^o)$ has rank  $\dim L$.
  \end{prop}
\begin{proof}%
\footnote{%The following 
This proposition is from  %unpublished lecture notes by P. Martin. 
\cite{MartinNRT}. A proof is also included here for the sake of self-containment.}
    Every simple factor in $M^o$ is extended by $L\simeq L^o$ below it 
    (recall that $M^o$ denotes the contravariant dual of $M$). 
  There is a map $\psi \in Hom_A(M, M^o)$ —that which kills the unique maximal proper submodule $\Mo$ and so makes the following diagram commute:
\[ 
\begin{tikzcd}
	0 && {\Mo} && M && L && 0 \\
	\\
	0 && {(\Mo)^o} && {M^o} && {L^o} && 0
	\arrow[from=1-1, to=1-3]
	\arrow[from=1-3, to=1-5]
	\arrow[from=1-5, to=1-7]
	\arrow[from=1-7, to=1-9]
	\arrow[from=3-9, to=3-7]
	\arrow[from=3-7, to=3-5]
	\arrow[from=3-5, to=3-3]
	\arrow[from=3-3, to=3-1]
	\arrow["\simeq"', from=1-7, to=3-7]
	\arrow["\psi"', from=1-5, to=3-5]
\end{tikzcd}\]
(or any scalar multiple thereof). No reduction is possible in the kernel, since this would require
factors appearing in the image below $L$, which $M^o$ does not have, as already noted. No enlargement
of the image is possible since this, correspondingly, requires factors above $L$ in $M.$ 
\end{proof}










==> tex/semisimplicity.tex <==

%




\ppm{We aim to prove below that}
Tower of Recollement (ToR) \cite{cox2006representation} is one of the axiomatic schemes where the argument in (\ref{pa:indicator}) can be lifted. In \cite{amm2019tonal} it is shown that the 2-tonal partition algebras with the idempotent \ca{$\W_n$} from (\ref{pa:U}) satisfy the ToR axioms—% of the tower of recollement. 
\ppm{[-this can't be right. Doesn't this `idempotent' have a hidden dependence on $n$!?]}
%\ppm{[-with what idempotent? It is not a tower but a tower each with an idempotent that is needed.]}\ca{[I think this is fixed now]}

\medskip 

\noindent
For $n \geqslant 0$, let $A_{n}$ be a family of finite-dimensional algebras, with idempotents $e_{n}\in A_{n}$. 
%Other examples of 
Here we briefly recall the ToR axioms {for such a family of pairs} from \cite{cox2006representation}:

\medskip 

\noindent 
A1) For each $n\geqslant2$, there is an isomorphism of algebras $e_nA_ne_n\cong A_{n-2}.$ 

\medskip 

%\ppm{[is the following an axiom or a property - a consequence of the axiom? I think the latter. So then say before:] Axiom A1 implies that [...?]}
Axiom A1 implies that there is a pair of functors associated with the isomorphism, 
$F_{n}: A_{n}$-mod $\rightarrow A_{n-2}$-mod and $G_{n}: A_{n}$-mod $\rightarrow A_{n+2}$-mod, defined by  $F_{n}(M)=e_{n} M$ and $G_{n-2}(N)=$ $A_{n} e_{n} \otimes_{e_{n} A_{n} e_{n}} N$. 

For each $n$
let $\Lambda_n$  be an indexing set for the isomorphism classes of simple $A_{n}$-modules. The globalisation functor $G_{n-2}$ takes projectives to projectives and hence induces an embedding of indexing set of simples $\Lambda_{n-2}\subset \Lambda_{n}$
(we may choose the sets so that this is an inclusion). 



For $m, n \in \mathbb{N}$ with $m-n$ even we set 
\[
\Lambda_{m}^{n}= \begin{cases}\Lambda_{n}\setminus \Lambda_{n-2} \subset \Lambda_m& \text { if }m \geqslant n \\ 
\emptyset & \text { if }  m < n\end{cases}
\]

\ppm{Define a partial order on $\Lambda_n$ by [???]}
%Let 
$\lambda \leqslant \mu$ if either $\lambda=\mu$ or $\lambda \in \Lambda_{n}^l$ and $\mu \in \Lambda_{n}^m$ with $l>m$. 



Set $e_{n, 0}=1\in A_{n}$, and for $1 \leqslant i \leqslant \frac{n}{2}$ define new idempotents in $A_{n}$ by letting $e_{n, i}$ be the image of $e_{n-2, i-1}$ under the isomorphism given in A1.

\medskip \medskip 

%For each $\lambda\in\Lambda_n$, 
Recall from \cite[Theorem 3.6]{cps}, a finite dimensional algebra $A$ is quasihereditary 
\ppm{with hereditary chain \[0\subset J_n\subset J_{n-1}\subset\dots\subset J_1=A\] [???]}
\ppm{[-I am very confused! It is red, but I don't remember writing this. And certainly it does not make any sense to me!]}
if and only if the the category  $A$-mod is a highest weight category with a poset $(\Lambda, \leqslant)$, where  $\Lambda$ is an indexing set for the isomorphism classes
of simple $A$-modules. See  \cite{KlucznikKoenig99} for more details about the equivalence of these two notions and construction of the standard modules from the hereditary chain and conversely. 
\ppm{[-this feels to me like it is running fast in the wrong direction. But we'll see. It might work. At this stage I suggest to concentrate on having a good statement and proof of Theorem.\ref{th:tor1}. Even if it makes the exposition very long. We can shorted later.]} \ca{[a proof of the correspondence? \ppm{--NO- see above} this is done in \cite{KlucznikKoenig99}]}




\medskip 

\noindent 
A2) The algebras $A_n$ are quasihereditary, 
\ppm{[-should we give the qh axioms? in the ToR paper the focus was introducing the new ToR axioms, but here all the axioms are relevant.]}\ca{[This is a good point, I think another option would be giving a reference]}\ppm{[then why not just give a reference for the ToR axioms!!? I just explained (tried to explain) why the different axioms should not be treated differently here.]}\ca{[Maybe the only justification here is qh algebras are more familiar than the axioms]}\ppm{[ok let's keep going. the test will be if the proof makes sense. for now add the reference you have in mind? - I note that there are several different formulations of qh, so a ref will at least tell which one you have in mind.]}
with heredity chain
\[
0 \subset \cdots \subset A_{n} e_{n, i} A_{n} \subset \cdots \subset A_{n} e_{n, 0} A_{n}=A_{n}.
\]
\ppm{[-I ca't guess what this means from the ellipsis.]}


\noindent
For each $\lambda\in \Lambda_n$, let $\mathcal{P}_n(\lambda)$ be the projective cover of the simple module $L_n(\lambda)$. The standard module $\Delta_n(\lambda)$ is defined to be the maximal quotient  of $\mathcal{P}_n(\lambda)$ with composition  factors $L_n(\mu)$ such that $\mu\leqslant\lambda$. 


The quasiheredity axiom (A2) implies that 
for each $\lambda\in\Lambda_n$ up to isomorphism
there is a unique \ppm{[I think maybe only unique up to isomorphism. And there are a lot of details to get clear. qh is not really just an algebra, but an algebra and a poset/heredity chain. otherwise not even unique up to isomorphism. the given chain is not maximal. ...]} standard module $\Delta_n(\lambda)$ with simple head $L_n(\lambda)$. 
\ppm{[-Let's just give the definition of standard module?]}



Besides $L_n(\lambda)$, all other composition factors of $\Delta_{n}(\lambda)$ are labelled by $\mu$ with $\mu<\lambda$. Note that for $\lambda \in \Lambda_{n}^{n}$, we have that $\Delta_{n}(\lambda) \cong L_{n}(\lambda)$.

%Further, t
The standard modules obey 
\[
G_{n}\left(\Delta_{n}(\lambda)\right) \cong \Delta_{n+2}(\lambda)
\] and 
\[
F_{n}\left(\Delta_{n}(\lambda)\right) \cong \begin{cases}\Delta_{n-2}(\lambda) & \text { if } \lambda \in \Lambda_{n-2} \\ 0 & \text { if } \lambda \in \Lambda_{n}\setminus\Lambda_{n-2}\end{cases}
\]

\medskip 

\noindent 
A3) For each $n$ there is an algebra inclusion $A_n\subset A_{n+1}.$


Associated with this inclusion A3 we have the induction $\Ind_n(M)=A_{n+1}\otimes_{A_n}M$ and restriction  $\Res_n$ functors. 

\noindent 
A4) For each $n \geqslant 1$ we have $A_{n} e_{n} \cong A_{n-1}$ as a left $A_{n-1}$, right $A_{n-2}$-bimodule.

Axiom A4 implies that \[\Res_{n+2}\left(G_{n}\left(\Delta_{n}(\lambda)\right)\right) \cong \Ind_n \Delta_{n}(\lambda)\] 
for each $\lambda\in \Lambda_n$.




The quasiheredity axiom (A2) also implies that the $\Delta$-modules (standard modules) form basis for the Grothendieck group of $A_n$. 

The {\em support} of an $A_n$-module $M$ 
\ppm{with a $\Delta$-filtration [???!]}
is defined to be the set  of labels $\lambda$ for which $\Delta_n(\lambda)$ occurs in the $\Delta$-filtration of $M$. 
We write $\Supp_n(M)$ for the support of $M$. 

\medskip 

\noindent 
A5) For each $\lambda \in \Lambda_n^{m}$ we have that $\Res_n\left(\Delta_{n}(\lambda)\right)$ has a $\Delta$-filtration and
\[
\Supp_{n-1}\left(\Res_n\left(\Delta_{n}(\lambda)\right) 
\;\subseteq\; 
\Lambda_{n-1}^{m-1} \sqcup \Lambda_{n-1}^{m+1}\right.
\]
%\ppm{[missing $n$???]}\ca{[fixed]}

\noindent 
A6) For each $\lambda \in \Lambda_{n}^{m}$ there exists $\mu \in \Lambda_{n+1}^{m-1}$ such that $\lambda \in \Supp_n\left(\Res \Delta_{n+1}(\mu)\right)$.

\medskip 

\newcommand{\lambdam}{\mu}

\begin{thm}  \label{th:tor1}
Let $(A_n , e_n), \; n\geq 0$ be a family of finite dimensional algebras and idempotents %\ppm{[right??Yes   :-) ]} 
satisfying the axioms $A1-A6$ of tower of recollement.  
Let  $\Delta_n(\lambda)$, $\lambda\in \Lambda_n$ denote  
the corresponding standard modules (as below A2). 
If $\Delta_n(\lambdam)$ is simple for each $n$   %and 
for 
each $\lambdam\in \Lambda_0$ then $A_n$ semisimple for all $n$.  
\end{thm} 


% 
%
\begin{proof}
\ppm{[This is a long, complicated proof, so it might be good to give a first sentence outlining the proof strategy? It would make sense to follow the (I-IV) structure of \ref{pa:indicator}, no? But so far what is here does NOT seem to me to do this!!]}

\ppm{We continue with the notation introduced with the axioms above.}
We write $|\lambda| = l$ if $\lambda\in\Lambda^l_n$ but $\lambda\notin\Lambda^m_n$ for any $m<l$. 

We break down the proof into three steps. In the first step we show that the result can be proven by induction on $|\lambda|$, 
\ppm{with $|\lambda|=$}\ca{0} \ppm{??? as base, [???]}
and then in the other two steps we perform the induction.\ca{[is it better now?]}\ppm{[I don't understand yet.]}


\noindent 
(I)
%If a module $M$ has a filtration by a set ${\mathcal T}$ of modules we say that it has a ${\mathcal T}$-filtration.
%%% ^ we don't need this here. said already now.
For any $n$ let $\Lambda(A_n)$ be an index set for simple $A_n$-modules corresponding to the set $\Lambda_n$ arising in the ToR setup above (below A1); and for $\lambda\in\Lambda(A_n)$. 
\ppm{[-this is not a sentence? I am lost.]}
 Let $ \pro_n(\lambda)$ be the projective cover of the simple $A_n$-module $L_n(\lambda)$. 
As for any finite-dimensional algebra over a field, to show $A_n$ is semisimple it is enough to show that  $ \pro_n(\lambda)$ is simple for each $\lambda\in\Lambda(A_n)$. Let $M$ be a finite dimensional $A_n$-module. Then 
$$
\dim \Hom( \pro_n(\lambda), M) \; =\; [M:L_n(\lambda)]
$$ 
where  $ [M:L_n(\lambda)]  $ denotes the 
multiplicity of $L_n(\lambda)$ in  %the composition  factor 
a composition series
of $M$. By the quasiheredity property (axiom A2) we have 
$\dim \Hom( \pro_n(\lambda), \Delta_n(\mu) )=[\Delta_n(\mu):L_n(\lambda)]\neq0$ 
\ppm{[-can we break this up so that the logic can be followed? is the middle element relevant here?]}\ca{[The point for the middle step is $[\Delta_n(\mu):L_n(\lambda)]\neq0$ if $\Hom(\Delta_n(\lambda), \Delta_n(\mu))\neq0$ and this is a property of qh algebras, but if you think this is not necessary we can delete it]}
if $\Hom(\Delta_n(\lambda), \Delta_n(\mu))\neq0$. But for quasihereditary algebras the projective covers are filtered by the standard modules, hence it is enough to show that there are no maps between the standard modules.    

\noindent
(II)
%Firstly n
Suppose $n$ is fixed. 
 Note that if $A_n$ is not semisimple then there must be a homomorphism
$\psi: \Delta_n(\mul) \rightarrow \Delta_n(\nul)$ for some 
distinct $\mul,\nul$;
in particular, by the quasiheredity axiom we have  $|\mul| > |\nul |$.
\ppm{[-I don't understand this yet.]}
And hence in particular some $\Delta_n(\nul) $ is not simple. 
So it is enough to prove that all $\Delta_n(\nul) $ are simple. 
We do this by induction on $|\nul|$.
\ignore{ 
Assuming $\delta \not\in \N_0$ then it 
is straightforward to eliminate cases with $|\mul| = |\nul | +1$,
so we consider $|\mul| > |\nul | +1$.
}

\noindent(III) 
%Consider
Recalling A3,
we will use the reciprocity
\beq \label{eq:FR--}
\Hom(\Ind \Delta_n(\mul), \Delta_{n+1}(\nul) ) \cong \Hom(\Delta_n(\mul) , \res \Delta_{n+1}(\nul) )
\eq 
%By A3 each $A_{n-1}$ is subalgebra of $ A_n$. %and by \ppm{[-delete this? Or possibly I have not understood.]}

By the 
Induction/Restriction rules (this is A5) 
(as indicated in Fig.\ref{fig:PnBratelli} for example), 
\ppm{[-what is this supposed to be an example of??? might be better if this reference is a separate sentence with some explanation?]}
we have 
\beq \label{eq:Indres--}
\Ind \Delta_n(\mul) \;\lleadsto \bigplus_{\rho \in \mul\pm 1} \Delta_{n+1}(\rho) ,
\qquad \hspace{.21in} 
\res \Delta_{n+1}(\mul) \;\lleadsto \bigplus_{\rho \in \mul\pm 1} \Delta_{n}(\rho) ,
\eq 
where $\lleadsto$ indicates 
$\Delta$-filtration \ppm{[-proof of filtration???]} and a covering set of 
filtration factors; 
and $\lambda\pm1$ indicates 
a set of factors with weights of rank between $|\lambda|+1$ and $|\lambda|-1$.
%So if we have $\psi: \SSS_n(\mul) \rightarrow \SSS_n(\nul)$ 
%then  ...

\ppm{[The following figure is not referenced or introduced until later!? maybe push it to that place? Or make it a fig? Or something.]}

\ppm{[something like this?:] The following schematic has a row of vertices indicating standard modules of $A_n$ (some with their labels shown); and a row for $A_{n+1}$ similarly. The precise vertical alignment is not significant, but the partition by vertical brown walls indicates partition according to `rank' $|\lambda|$,
with lower ranks to the left. [BUT this does not seem to work, since the axiomatic setup as in A5 forbids same ranks between adjacent algebras!?!?!?!] The black edges then indicate restriction (on the left) and induction (on the right).
}
\beq  \label{eq:FR111--}
\includegraphics[width=10cm]{figs/FrobRecip111.eps}
\eq

\noindent
(IV)
So now suppose for an induction that modules 
$\Delta_n(\mu)$
of ranks $|\mu|$ up to $l$ are simple \ppm{for all $n$???}.
The base is exactly the hypothesis \ppm{of ???? [the last hypothesis was quite a while ago!]}.
This implies no maps $\psi$ 
into $\Delta_n(\mu)$ (apart from self-isomorphism), 
so then in particular
for every $\mu$ of rank $|\mu| =l$ we have 
$ \Hom(\Ind \Delta_n(\mul), \Delta_{n+1}(\mu) ) =0$ for all $\mul$ of rank at least $|\mu|+2$, by (\ref{eq:Indres--}) and Schur's Lemma.
But suppose (for a contradiction, in the inductive step to $l+1$) some 
$\Delta_n(\nu)$ with 
$\nu$ of rank $l+1$ 
is not simple, and hence has a map in, from $\Delta_n(\lambda)$ say. 
See the figure in (\ref{eq:FR111--}) (and cf. (\ref{eq:FR111})).
The factors in any $\res \Delta_n(\mu)$ as above are either in their own block by 
the inductive assumption, or of equal rank to $\nu$ and hence
(cf. (\ref{pa:globloc101}))
not involved
in extensions with $\Delta_n(\nu)$,
and by A6 for a suitable $\mu$ they include $\Delta_n(\nu)$. 
Thus there is a map in 
$  \Hom(\Delta_n(\mul) , \res \Delta_{n+1}(\mu) )  $. 
This then contradicts (\ref{eq:FR--}). 
We deduce that every $\Delta_n(\nu)$ with 
$\nu$ of rank $l+1$ is simple, which completes the inductive step.
\end{proof}


\ca{[The following is a proposal of an alternative form of the  theorem \ref{th:tor1}]}


For $n \geq 0$, let $A_{n}$ be a family of finite-dimensional algebras, with idempotents $e_{n}\in A_{n}$. We start by imposing five conditions on $(A_n,e_n)$ that allow us to test the semisimplicity of each $A_n$ by checking the simplicity of a relatively small set of modules.


\noindent
A-I) For each $n\geq1$  we have $e_{n}A_{n}e_{n}\cong A_{n-1}$ as algebras.   

\noindent
Axiom AI implies that there is a pair of functors associated with the isomorphism, 
$F_{n}: A_{n}$-mod $\rightarrow A_{n-1}$-mod and $G_{n}: A_{n}$-mod $\rightarrow A_{n+1}$-mod, defined by  $F_{n}(M)=e_{n} M$ and $G_{n-1}(N)=$ $A_{n} e_{n} \otimes_{e_{n} A_{n} e_{n}} N$.


\noindent
For each $n$
let $\Lambda_n$  be an indexing set for the isomorphism classes of simple $A_{n}$-modules. The globalisation functor $G_{n-1}$ takes projectives to projectives and hence induces an embedding of indexing set of simples $\Lambda_{n-1}\subset \Lambda_{n}$
(we may choose the sets so that this is an inclusion).


\noindent
A-II) Each $A_n$ is quasiherditary\ca{[I understand we discuss the proper way of recalling the qh axiom, but for now the aim is to see if the whole theorem makes sense]}. 
Let 
$\{\Delta_n(\lambda):\lambda\in \Lambda_n\}$ be a complete set of standard $A_n$-modules with the partial order  $\leqslant$ on $\Lambda_n$ induced by the quasiherdity property.  


\noindent
We write $|\lambda| = n$ if $\lambda\in\Lambda_n\setminus\Lambda_{n-1}$.


\noindent
A-III) For each $n$ there is an algebra inclusion $A_n\subset A_{n+1}$. 

\noindent
Associated with the above inclusion we have the induction $\Ind_n(M)=A_{n+1}\otimes_{A_n}M$ and restriction  $\Res_n$ functors.


\noindent
A-IV) For each $n$ we have
\beq \label{eq:Indrescore}
\Ind_n \Delta_n(\mul) \;\lleadsto \bigplus_{\rho \in \mul\pm 1} \Delta_{n+1}(\rho) ,
\qquad \hspace{.21in} 
\Res_{n+1} \Delta_{n+1}(\mul) \;\lleadsto \bigplus_{\rho \in \mul\pm 1} \Delta_{n}(\rho) ,
\eq 
where $\lleadsto$ indicates 
$\Delta$-filtration and a covering set of 
filtration factors; and $\lambda\pm1$ indicates 
a set of factors with weights of rank between $|\lambda|+1$ and $|\lambda|-1$.

\noindent
A-V) For each $\rho\in \Lambda_n\setminus\Lambda_{n-1}$ there is a $\mu\in \Lambda_{n-1}\setminus\Lambda_{n-2}$ such that $\Delta_n(\rho)$ is a factor of $\Res(\Delta_{n+1}(\mu))$ in the $\Delta$-filtration.

\begin{thm}  \label{th:cor}
Let $(A_n , e_n), \; n\geq 0$ be a family of finite dimensional algebras and idempotents
satisfying the axioms $AI-AV$.  
Let  $\Delta_n(\lambda)$, $\lambda\in \Lambda_n$ denote  
the corresponding standard modules (as below AII). 
If $\Delta_n(\lambdam)$ is simple for each $n$   %and 
for 
each $\lambdam\in \Lambda_0$ then $A_n$ semisimple for all $n$.  
\end{thm} 

==> tex/semisimplicity0.tex <==


\section{On generalising the spine-simplicity criterion (\ref{pa:indicator}) for semisimplicity}  
%$\;$ 

In \S\ref{ss:maintheo} we  show  %%will see 
that a  %generalisation 
modification of the argument in (\ref{pa:indicator}) applies to 
the tonal case. 
This raises the question of the appropriate level of generality for such arguments. For our purposes here 
%we have what we need
the modification is sufficient,
but in this Section we consider a couple of standard axiomatic 
frameworks to which the argument lifts. 

In (\ref{pa:indicator})(I) we assume 
standard properties of standard modules. This is safe, in the 
sense that they hold in our cases, and good for brevity,
but not so helpful for 
exposition. So in large part the exercise here is to set up the
key properties explicitly. 




